Resource Sharing Through Multi-Round Matchings

Applications such as employees sharing office spaces over a workweek can be modeled as problems where agents are matched to resources over multiple rounds. Agents' requirements limit the set of compatible resources and the rounds in which they want to be matched. Viewing such an application as a multi-round matching problem on a bipartite compatibility graph between agents and resources, we show that a solution (i.e., a set of matchings, with one matching per round) can be found efficiently if one exists. To cope with situations where a solution does not exist, we consider two extensions. In the first extension, a benefit function is defined for each agent and the objective is to find a multi-round matching to maximize the total benefit. For a general class of benefit functions satisfying certain properties (including diminishing returns), we show that this multi-round matching problem is efficiently solvable. This class includes utilitarian and Rawlsian welfare functions. For another benefit function, we show that the maximization problem is NP-hard. In the second extension, the objective is to generate advice to each agent (i.e., a subset of requirements to be relaxed) subject to a budget constraint so that the agent can be matched. We show that this budget-constrained advice generation problem is NP-hard. For this problem, we develop an integer linear programming formulation as well as a heuristic based on local search. We experimentally evaluate our algorithms on synthetic networks and apply them to two real-world situations: shared office spaces and matching courses to classrooms.

==> hardness.tex <==
%\newcommand{\setc}{\mathcal{Z}}

%\section{Complexity of \msmrm{} and \agmrm}
\section{Complexity of Max Versions}
\label{sec:complexity}
Our hardness results for \agmrm{} and \msmrm{} follow.

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm:hardness}
The \agmrm{} problem is NP-hard when there is just one
agent~$x_i$ such that~$\rho_i > 1$.
%Further, if the constraint on the number of rounds must be
%satisfied, then there is no polynomial time algorithm for
%finding a solution that violates the budget
%for each agent by a factor $o(\log{m})$, where $m$ is the
%number of resources, 
%unless \textbf{P} = \cnp. 
\end{theorem}

\noindent
\textbf{Proof outline.}~We use a reduction
from the Minimum Set Cover (MSC) problem
which is known to be \cnp-complete
\cite{GareyJohnson79}.
%Here, we only provide the construction of the
%\agmrm{} instance given the MSC instance. The proof that there exists a
%solution to the MSC problem iff there exists a solution to the \agmrm{}
%problem is in the supplement. 
Consider an instance of MSC consisting of a
set~$U=\{z_1,z_2,\ldots, z_t\}$, a collection~$\setc=\{A_1,A_2,\ldots,
A_q\}$ of $q$ subsets of~$U$, and an integer~$\alpha\le|\setc|$.
%is there a
%subcollection ~$\setc'\subseteq\setc$ such that~$|\setc'|\le\alpha$
%and~$\bigcup_{Z\in \setc'}Z = U$?
We will construct an instance of \agmrm{} as
follows. Let~$t =|U|$.  Let degree of an element~$z\in U$, denoted
by~$\deg(z)$, be the number of sets in~$\setc$ which contain $z$.  For
each~$z_j\in U$, we create~$\deg(z_j)$ resources~$\rset_j=\{y_j^h\mid
z_j\in A_h\}$. Thus, the resource set is~$\rset = \bigcup_{z_j\in
U}\rset_j$. For each~$\rset_j$, we create a set of agents~$\agset_j =
\{x_j^1,x_j^2,\ldots\}$, where~$|\agset_j| = t\cdot\deg(z_j)-1$. For
each~$z_j\in U$, we have an edge for every~$x\in \agset_j$ and~$y\in
\rset_j$. Finally, we add a special agent~$x^*$ with edges to all
resources. The set of agents is~$\agset=\bigcup_{z_j\in
U}\agset_j\cup\{x^*\}$. For each~$x\ne x^*$, there are no labels on the
edges that are incident on $x$. For each edge~$\{x^*,y_j^h\}$, we assign a
single label~$c_h$. Each label has cost~$1$. This completes the
construction of~$G_R$. For~$x^*$, the budget $\beta^*=\alpha$, which is the
budget for the MSC instance, and for all other agents, the budget is~$0$.
The number of rounds for~$x^*$,~$\rho^*=t$ and for the rest of the
agents~$x_i\ne x^*$,~$\rho_i=1$. For all agents~$x_i$,
$K_i=\{1,\ldots,t\}$. 
This completes the construction of a
\msagmrm{} instance.
A correctness proof for this reduction appears in the supplement. \qed
%%%%%%%%%%%%%%%%%%%%
\fi
%It can be seen that this construction can be done
%in polynomial time.\qed

\iffalse
%%%%%%%%%%%%%%%%%% Moved elsewhere %%%%%%%%%%%%%
\begin{theorem}\label{thm:max_sat_agents_npc}
\msmrm{} is \cnp-hard even when the number of rounds ($k$) is 3.
\end{theorem}

\noindent
\textbf{Proof outline:}~
To prove \cnp-hardness, we use a reduction from the Minimum Vertex Cover
Problem for Cubic graphs, which we denote as \mvcc{}.
A definition of this problem is as follows: given
an undirected graph $H(V_H, E_H)$ where the degree of each node is 3
and an integer $h \leq |V_H|$, is there a vertex cover of size at most $h$ for $H$?
%(i.e., a subset $V'_H \subseteq V_H$
%such that $|V'_H| \leq h$, and for each edge $\{x,y\} \in %E_H$, at least
%one of $x$ and $y$ is in $V'_H$)?
It is known that \mvcc{} is \cnp-complete \cite{GareyJohnson79}.
Given an instance $I$ of \mvcc{} consisting of graph $H(V_H, E_H)$
and integer $h \leq |V_H|$, we produce an instance $I'$ of \msmrm{}
where the number of rounds = 3, with some agents requiring just one
round while others need three rounds.
The details of the reduction and its proof of correctness appear in the supplement. \hfill$\Box$
%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi



==> mrm_algorithm.tex <==
\section{An Efficient algorithm for \mrm{}}
\label{sec:mrm_poly}
We now present a polynomial time algorithm for \mrm.
The basic idea is to reduce the problem to the maximum
matching problem on a larger graph.
The steps of our algorithm \algmrm{} for \mrm{} are shown
in Figure~\ref{fig:alg-mrma-prb}.
An example to illustrate the construction used in the algorithm
is given in the supplement.

\begin{figure}[ht]
\rule{\columnwidth}{0.01in}
{\small
    \begin{enumerate}[leftmargin=*]
\item Given compatibility graph $G(X, Y, E)$,
create a new bipartite graph $G'(V', W', E')$ as follows.
To begin with, the sets  $V'$, $W'$ and $E'$ are all empty.
\begin{enumerate}[leftmargin=*]
      \item For each resource node $y_j \in Y$, add $k$ nodes denoted
      by $y_j^t$, where $t = 1, 2, \ldots, k$, to $W'$.

      \item For each agent $x_i \in X$ with $\rho_i = 1$:
      (i) Add a new node $x_i^1$ to $V'$.
      (ii) For each edge $\{x_i, y_j\} \in E$ and $t \in K_i$, add the edge
      $\{x_i^1, y_j^t\}$ to $E'$.

      \item For each agent $x_i \in X$ with  $\rho_i \geq 2$:
            (i) For each $t \in K_i$, add a node denoted by $x_i^t$ to $V'$.
            (ii) Add $q_i = |K_i|- \rho_i$ ``dummy-resource" nodes, denoted
            by $z_i^{\ell}$, where $\ell = 1, 2, \ldots, q_i$, to $W'$.
            (iii) For each edge $\{x_i, y_j\} \in E$ and each $t \in K_i$,
             add the edge $\{x_i^t, y_j^t\}$ to $E'$.
            (iv) For each node $x_i^t$, add the
            $|K_i|- \rho_i$ edges $\{x_i^t, z_i^{\ell}\}$,
            $1 \leq \ell \leq |K_i|-\rho_i$, to $E'$.
   \end{enumerate}
\item Find a maximum matching $M'$ in $G'(V', W', E')$.
\item If $M'$ does \emph{not} include all the nodes in $V'$, then
      print ``No Solution" and \textbf{stop}.
      \item Compute a collection of matchings $M_1$, $M_2$, $\ldots$, $M_k$, for
$G$ as follows. These matchings are initially empty.
For each edge $e \in M'$ that does \emph{not} use a
      dummy resource, do the following:
                (a) Let $x_i^{t}$ and $y_j^{\ell}$ denote the
                      end points of $e$.
                (b) Add the edge $\{x_i, y_j\}$ to $M_{\ell}$.
\end{enumerate}
}
\caption{Steps of \algmrm{} for \mrm{}}
\label{fig:alg-mrma-prb}
\rule{\columnwidth}{0.01in}
\end{figure}

The following result establishes the correctness
and running time of \algmrm.

\begin{theorem}\label{thm:alg_mmra_prb_correct}
(i) There is a solution to the \mrm{} instance iff the graph
$G'$ constructed in Step~1 of Algorithm 
\algmrm{} has a matching of size $|V'|$.
(ii) The running time of the algorithm is
$O(k^{3/2}|E| \sqrt{|X|+|Y|})$.
\end{theorem}

\noindent
\textbf{Proof outline:} Our proof of Part~(i) involves showing
that there is a solution to an \mrm{} instance 
(consisting of matchings $M_1$, $M_2$, $\ldots$, $M_k$)
iff there is a matching $M'$ of $G'$ that matches all the nodes in $V'$. 
To prove Part~(ii), we show that graph $G'$ has
$O(k(|X|+|Y|)$ nodes and $O(k|E|)$ edges and
use the fact that for any bipartite graph $H(V_H, E_H)$,
a maximum matching can be found in
$O(|E_H| \sqrt{|V_H|})$ time \cite{CLRS-2009}.
See the supplement for details.\hfill$\Box$

 




==> rawlsian.tex <==
\newcommand{\ord}{\pi}
\newcommand{\Fg}{F^>}
\section{Rawlsian social welfare}
\label{sec:rawlsian}
Let~$\gamma_i(\mbsoln)$ denote the number of rounds in which agent~$x_i$ is
matched in a multi-round solution~$\mbsoln$. The minimum satisfaction ratio
for~$\mbsoln$ is defined as~$\min_{i}\gamma_i(\mbsoln)/\rho_i$. We show the
following result.
%%
\begin{theorem}\label{thm:rawlsian}
There exists a reward function for which the optimal multi-round solution
satisfies Rawlsian social welfare, i.e., it maximizes the minimum
satisfaction ratio over all agents. Further, this reward function satisfies
the diminishing rewards property, and therefore, the optimal solution can
be computed in polynomial time.
\end{theorem}
%%
\noindent
The reward function is constructed as follows: 
\begin{enumerate}[leftmargin=*]
\item Let~$F=\big\{k_1/k_2\mid k_1,k_2\in\{1,\ldots,k\}\big\}\cup\{0\}$.
\item Let~$\ord: F\rightarrow\{1,\ldots,|F|\}$ correspond to the index of
each element in~$F$ when sorted in descending order.
\item For each~$q\in F$, $\xi(q)=(nk)^{\ord(q)}/(nk)^{|F|}$, where~$n$ is
the number of agents and~$k$ is the number of rounds. Note that
each~$\xi(q)\in(0,1]$.
\item The incremental reward~$\delta_i(\ell)$ for an agent~$x_i$ for
the~$\ell$th matching is defined
as~$\delta_i(\ell)=\xi\big((l-1)/\rho_i\big)$.
\end{enumerate}
%%
\begin{lemma}
For each agent~$x_i$, the incremental reward~$\delta_i(\ell)$ is monotone
non-increasing in~$\ell$, and therefore,~$\mu_i(\cdot)$ satisfies
diminishing returns property.
\end{lemma}
%%
\begin{proof}
By definition, for~$\ell=1,\ldots,\rho_i-1$,~$\delta_i(\ell)/\delta_i(\ell+1)=
\xi\big((\ell-1)/\rho_i\big)/\xi\big(\ell/\rho_i\big)\ge nk > 1$, by noting
that~$\pi(\ell/\rho_i)-\pi((\ell+1)/\rho_i)\ge1$. Hence proved.
\end{proof}
%%
\noindent
%%For~$q\in F$, let~$\Fg(q)=\{q'\mid q'\in F \text{ and } q'>q\}$.
For an agent~$x_i$ and~$q\in F$, let~$\Fg_i(q)=\{\ell\mid 0\le\ell\le\rho_i
\text{ and } \ell/\rho_i>q\}$. We will now show that the incremental
reward~$\delta_i(\ell)$ obtained by agent~$x_i$ for matching~$\ell$ is
greater than the sum of all incremental rewards~$\delta_{i'}(\ell')$, for
all agents~$x_{i'}$, $i'\ne i$ and for all~$\ell'$
satisfying~$\ell'/\rho_{i'}>\ell/\rho_i$.
%%
\begin{lemma}\label{lem:cost}
For any agent~$x_i$ and non-negative
integer~$\ell\le\rho_i$,~$\delta_i(\ell)>\sum_{i'=i}\sum_{\ell'\in
\Fg_{i'}(\ell/\rho_i)}\delta_{i'}(\ell')$.
\end{lemma}
%%
\begin{proof}
For any~$\ell'\in \Fg_{i'}(\ell/\rho_i)$, note that
$\ell/\rho_i<\ell'/\rho_{i'}$.
Hence,~$\pi(\ell/\rho_i)-\pi(\ell'/\rho_{i'})\ge1$. This implies
that~$\delta_i(\ell)/\delta_{i'}(\ell') =
\xi\big((\ell-1)/\rho_i\big)/\xi\big((\ell'-1)/\rho_{i'}\big)\ge nk$.
Since~$\rho_{i'}\le k$, there are at most~$k$~$\delta_{i'}(\ell')$ terms
per~$i'$. Since there are at most~$n-1$ agents~$x_{i'}$,~$i'\ne i$, it
follows that there are at most~$(n-1)k$ terms~$\delta_{i'}(\ell')$ in
total. Therefore,~$\sum_{i'=i}\sum_{\ell'\in
\Fg_{i'}(\ell/\rho_i)}\frac{\delta_{i'}(\ell')}{\delta_{i}(\ell)}<1$.
\end{proof}
%%
\noindent
\textbf{Proof of Theorem~\ref{thm:rawlsian}.}
The proof is by contradiction. Suppose~$\mbsoln^*$ is an optimal solution
given the reward function defined above. We will show that if there exists
a solution~$\mbsoln$ with minimum satisfaction ratio greater than that
of~$\mbsoln^*$, then, the
benefit~$\totreward(\mbsoln)>\totreward(\mbsoln^*)$, contradicting the fact
that~$\mbsoln^*$ is an optimal solution. Let~$q(\mbsoln^*)$
and~$q(\mbsoln)$ denote the minimum satisfaction ratio in~$\mbsoln^*$
and~$\mbsoln$.

We recall that the benefit function for~$\mbsoln$ can be written
as~$\totreward(\mbsoln)=\sum_{i=1}^n\sum_{\ell=1}^{\gamma_i(\mbsoln)}
\delta_i(\ell)$. For each~$i$, the~$\delta_i(\ell)$ terms can be
partitioned into three blocks: (i)~$D_1(\mbsoln)=\{(i,\ell)\mid \forall
i,~\ell/\rho_i\le q(\mbsoln^*)\}$, (ii)~$D_2(\mbsoln)=\{(i,\ell)\mid
\forall i,~q(\mbsoln^*)<\ell/\rho_i\le q(\mbsoln)\}$ and
(ii)~$D_3(\mbsoln)=\{(i,\ell)\mid \forall i,~\ell>q(\mbsoln)\}$. We can
partition the terms corresponding to~$\totreward(\mbsoln^*)$ in the same
way, denoted by~$D_1(\mbsoln^*)$ and~$D_2(\mbsoln^*)$. Note that since
every~$x_i$ has a satisfaction ratio of at least~$q(\mbsoln^*)$ in
both~$\mbsoln^*$ and~$\mbsoln$, all the terms with~$\ell/\rho_i\le
q(\mbsoln^*)$ will be present. Therefore,~$D_1(\mbsoln^*)=D_1(\mbsoln)$.

In~$\mbsoln^*$, let~$x_{i'}$ be the agent for which the satisfaction ratio
is~$q(\mbsoln^*)$. There are no~$(i',\ell)$ terms in~$D_2(\mbsoln^*)$ while
for every agent~$x_i$, all~$(i,\ell)$ terms
satisfying~$q(\mbsoln^*)<\delta_i(\ell)\le q(\mbsoln)$ are present
in~$D_2(\mbsoln)$. Therefore,~$D_2(\mbsoln^*)\subset D_2(\mbsoln)$.
%%
\begin{align*}
\totreward(\mbsoln)-\totreward(\mbsoln^*) = & 
\sum_{(i,\ell)\in D_2(\mbsoln)}\delta_i(\ell) +
\sum_{(i,\ell)\in D_3(\mbsoln)}\delta_i(\ell) -
\sum_{(i,\ell)\in D_2(\mbsoln^*)}\delta_i(\ell) -
\sum_{(i,\ell)\in D_3(\mbsoln^*)}\delta_i(\ell) \\
& >
\sum_{(i,\ell)\in D_2(\mbsoln)}\delta_i(\ell) -
\sum_{(i,\ell)\in D_2(\mbsoln^*)}\delta_i(\ell) -
\sum_{(i,\ell)\in D_3(\mbsoln^*)}\delta_i(\ell) \\
\end{align*}
%%
Now, let~$(i',\ell')=\argmin_{(i,\ell)\in D_2(\mbsoln)\setminus
D_2(\mbsoln^*)} \ell/\rho_i$. Also, recalling that~$D_2(\mbsoln^*)\subset
D_2(\mbsoln)$,
%%
\begin{align*}
\totreward(\mbsoln)-\totreward(\mbsoln^*) & >
\sum_{(i,\ell)\in D_2(\mbsoln)}\delta_i(\ell) -
\sum_{(i,\ell)\in D_2(\mbsoln^*)}\delta_i(\ell) -
\sum_{(i,\ell)\in D_3(\mbsoln^*)}\delta_i(\ell) \\
& > \delta_{i'}(\ell') -
\sum_{(i,\ell)\in D_3(\mbsoln^*)}\delta_i(\ell) > 0\\
\end{align*}
%%
The inequality follows from Lemma~\ref{lem:cost}.
\qed





==> scratch.tex <==
\section{Additional Material for Section~\ref{sec:experiments}}
\label{sup:sec:experiments}
Due to space limitation, we could not include the results of our experiments
with the \pv{} dataset in the context of \problemrone{} (\agmrm{} with
requirement at least one) in the main paper. Those results are in
Figure~\ref{mrmar1_pv}. The experiment design is same as that explained
for Figure~\ref{mrmar1} (first three plots) with regard to \cc{}
experiments. We note that the results indicate that among all
restrictions, activity preferences of children is the one that leads to the
most reduction in the number of rounds required when relaxed. Also, we note
that, unlike in the \cc{} case, relaxation of combinations of attributes
does not have much effect compared to relaxation of the activity preference
alone..
%%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=.32\columnwidth]{figures/mrmar1_pv_1.pdf}
    \includegraphics[width=.32\columnwidth]{figures/mrmar1_pv_2.pdf}
    \includegraphics[width=.32\columnwidth]{figures/mrmar1_pv_3.pdf}
    \caption{\problemrone{} results for \pv{}. In
the \pv{} plots, for relaxations beyond the values on the $x$-axes,
the results are unchanged.}
\label{mrmar1_pv}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.5\columnwidth]{figures/mrma_heuristic_pv.pdf}
    \caption{\SAproblem{} results for \pv{}. The graph that compares \SAproblem{} to \ilpproblem{} is not presented since the runtime of  \ilpproblem{} on the \pv{} dataset is too long and not practical. }
\label{mrmar1_pv_2}
\end{figure}
%% to find optimal solutions for both \problem{} and \problemprb{} problems.
%% Also, we present a heuristic algorithm which combines a greedy approach
%% with a local search method to generate solutions of good quality in a
%% reasonable amount of time.
\iffalse
%%%%%%%%%%%%% These lines are now in the file named %%%%%%%
%%%%%%%%%%%%%% experiments.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[scale=0.5]{figures/school_k.png}
\begin{itemize}
    \item Based on School vacations graph
    \item x axis is the agents with demand in {5,10,15,20} rest are with demand of 2 matchings.
    \item different values of k for ilp and greed heuristics.
    \item 10 datapoints for different percents.
    \item high requirement agents are chosen randomly 100 times and average is calculated.
    \item graph is after relaxation with budget of 2.
    
\end{itemize}


\includegraphics[scale=0.5]{figures/school_time.png}
\begin{itemize}
    \item runtimes for greedy and ilp
    \item using cbc solver. tried also gurobi which considered as state of the art.
    
\end{itemize}
\includegraphics[scale=0.5]{figures/class_k.png}
\begin{itemize}
    \item Same definitions but for courses and classes
\end{itemize}


\includegraphics[scale=0.5]{figures/class_times.png}
\begin{itemize}
    \item Same definitions but for courses and classes
\end{itemize}



\includegraphics[scale=0.5]{figures/relax_course_k_1.png}
\begin{itemize}
    \item Previous graph for comparison, please ignore.
\end{itemize}

\includegraphics[scale=0.5]{figures/relax_course_k_1_2.png}
\begin{itemize}
    \item Relaxing 0.0,0.2,0.4,0.6,0.8 or 1.0 of the constraints for each relevant attribute.
    \item Remove agents with no edges in the beginning.
    \item save runtimes as well
    \item choose k by using algorithm of at least one.
    
\end{itemize}

\includegraphics[scale=0.5]{figures/random_k.png}

\begin{itemize}
    \item Random graphs. agents are chosen among large initial set  such that they will have at least 1 edge.
    \item No requirement from the resources.
    \item 4 data points, 100,0.75,0.5,0.25
    \item run massively in parallel, 1000 times per option.
    
\end{itemize}

\includegraphics[scale=0.5]{figures/local_search.png}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi


%%%%%%%%%%%%%% From here on, all the material in this file %%%%%%%%
%%%%%%%%%%%%%% has been commented out.                  %%%%%%%%%%%
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Material for 
Section~\ref{sec:methods_per_round_budget}}

\medskip

\subsection{A Simpler ILP for \maxmrm{}}
\label{sup:sse:simpler_ilp}

Section~\ref{sec:general_ilp} presented an ILP for \maxagmrm{}.
Here, we present a simpler ILP for \maxmrm{} where 
the compatibility graph $G(X, Y, E)$ is given.

\smallskip

\noindent
\textbf{ILP Formulation:}~ 

\smallskip

\noindent
\underline{\textsf{Variables:}} 
\begin{itemize}
\item For each agent $x_i$, let $A_i$ denote the
set of resources with which $x_i$ is compatible;
that is, $A_i = \{y_j ~:~ \{x_i, y_j\} \in E\}$, $1 \leq i \leq n$.
For each agent $x_i$ and each resource $y_j \in A_i$,
we have $k$ \{0,1\}-variables
denoted by $a_{ijr}$, where $1 \leq i \leq n$, $1 \leq j \leq m$ and
$1 \leq r \leq k$.
The interpretation is that  $a_{ijr}$ is 1 iff agent $x_i$ is matched
to resource $y_j$ in round $r$.

\item For each agent $x_i$, we have a non-negative integer
variable $\eta_i$ which gives the number of rounds
in which $x_i$ is matched.

\item For each agent $x_i$, we have a \{0,1\}-variable $s_i$
that is 1 iff agent $x_i$'s requirement is satisfied.
\end{itemize}

\smallskip

\noindent
\underline{\textsf{Objective:}}~ Maximize~~
$\sum_{i=1}^{n} s_i$.

\smallskip

\noindent
\underline{\textsf{Constraints:}} 

\begin{itemize} [leftmargin=*,noitemsep,topsep=0pt]
\item For each agent $x_i$, the number of rounds
in which $x_i$ is matched should equal $\eta_i$.
This constraint can be expressed as
\begin{equation}
\sum_{r=1}^{k}\: \sum_{y_j \in A_i} a_{ijr} ~=~ \eta_i, ~~1 \leq i \leq n
%\label{eqn:v1_agent_deg}
\end{equation}

\item Each agent $x_i$ is matched to a resource \emph{at most once}
in each round.  This constraint can be expressed as
\begin{equation}
\sum_{y_j \in A_i}\: a_{ijr} ~\leq~ 1, ~~1 \leq i \leq n,~~ 1 \leq r \leq k
\end{equation}

\item For each resource $y_j$, let $B_j$ denote the set of agents
with which $y_j$ is compatible, $1 \leq j \leq m$;
that is, $B_j = \{x_i ~:~ \{x_i, y_j\} \in E\}$, $1 \leq j \leq m$.
In each round, each resource must be matched to an agent
\emph{at most} once. 
This constraint can be expressed as
\begin{equation}
\sum_{x_i \in B_j} a_{ijr} ~\leq~ 1, ~~
               1 \leq j \leq m,~~ 1 \leq r \leq k 
%\label{eqn:v1_res_deg}
\end{equation}

\item The rounds in which an agent $x_i$ is matched
must be in $K_i$. The corresponding constraint is:
\begin{align}
    a_{ijr} ~=~ 0, ~~ r \not\in K_i,~ 1 \leq j \leq m,~
     1 \leq i \leq n
\end{align}

\item Variable $s_i$ to be 1
iff agent $x_i$ was matched
in at least $\rho_i$ rounds. The following constraints,
which must hold for each $i$, $1 \leq i \leq n$, ensure this
condition.
\begin{eqnarray*}
k\,s_i ~\leq~ \eta_i - \rho_i + k \\
k\,s_i ~\geq~ \eta_i - \rho_i + 1 
\end{eqnarray*}

\item $a_{ijr} \in \{0,1\}$, 
$1 \leq i \leq n$,~ $1 \leq j \leq m$,~ $1 \leq r \leq k$.
\end{itemize}

\medskip

\noindent
\underline{\textsf{Obtaining a Solution:}} After solving
the ILP, for each variable $a_{ijr}$ which is set to 1 in the
solution, we match agent $x_i$ with resource $y_j$ in round $r$.
%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%\input{ilp_many_requirement_matching}

\iffalse
%%%%%%%%%%%%%%%%%%%%%%
\medskip
We now present an example to illustrate the above ILP
formulation.

\noindent
\textbf{Example:} In the compatibility graph shown below,
we have an agent $x_3$ which must appear in at least two rounds
of matching. 
(Recall from Section~\ref{sec:general_ilp} that for each agent
$x_i$, $A_i$ is the set of resources to which $x_i$
can be matched. Likewise, for each resource
$y_j$, $B_j$ is the set of agents to which $y_j$
can be matched.)

\bigskip

\begin{center}
\begin{minipage}{0.3\textwidth}
\input{graph_one.pdf_t}
\end{minipage}
\hspace*{0.1in}
\begin{minipage}{0.4\textwidth}
\begin{itemize}
\item Let $k = 2$.
\item Let $\rho_1 = 1$, $\rho_2 = 1$ and $\rho_3 = 2$.
\item $A_1 = \{y_1\}$, $A_2 = A_3 = \{y_1, y_2\}$.
\item $B_1 = \{x_1, x_2, x_3\}$ and $B_2 = \{x_2, x_3\}$.
\end{itemize}
\end{minipage}
\end{center}

\medskip

\noindent
The ILP for the above problem instance is as follows.

\bigskip

\noindent
\underline{\textsf{Variables:}}~ 
$a_{1,1,1}$, $a_{1,1,2}$,
$a_{2,1,1}$, $a_{2,1,2}$,
$a_{2,2,1}$, $a_{2,2,2}$,
$a_{3,1,1}$, $a_{3,1,2}$,
$a_{3,2,1}$ and $a_{3,2,2}$.
(Each of these variables takes on a value from $\{0,1\}$.
The significance of variable $a_{ijr}$ is that it takes on the
value 1 iff agent $x_i$ is assigned resource $y_j$ in round $r$.)

\bigskip

\noindent
\underline{\textsf{Constraints:}} 

\begin{itemize}
\item For Agent $x_1$: (i) $a_{1,1,1} + a_{1,1,2} ~\geq~ 1$,~
(ii) $a_{1,1,1} \leq 1$~ and (iii) $a_{1,1,2} \leq 1$. 
(The last two constraints can be omitted since the fact
that each variable takes on a value from $\{0,1\}$
implies each of the last two constraints.)

\item For Agent $x_2$: (i) $a_{2,1,1} + a_{2,2,1} 
                        +a_{2,1,2} + a_{2,2,2} ~\geq~ 1$,~
                (ii) $a_{2,1,1} + a_{2,2,1} ~\leq~ 1$~ and 
                (iii) $a_{2,1,2} + a_{2,2,2} ~\leq~ 1$.

\item For Agent $x_3$: (i) $a_{3,1,1} + a_{3,2,1} 
                        +a_{3,1,2} + a_{3,2,2} ~\geq~ 2$,~
                       (ii) $a_{3,1,1} + a_{3,2,1} ~\leq~ 1$ and
                       (iii) $a_{3,1,2} + a_{3,2,2} ~\leq~ 2$.

\item For Resource $y_1$: 
    \begin{description}
      \item{(a)} $a_{1,1,1} + a_{2,1,1} + a_{3,1,1} ~\leq~ 1$
      \item{(b)} $a_{1,1,2} + a_{2,1,2} + a_{3,1,2} ~\leq~ 1$
    \end{description}

\item For Resource $y_2$: 
    \begin{description}
      \item{(a)} $a_{2,2,1} + a_{3,2,1} ~\leq~ 1$
      \item{(b)} $a_{2,2,2} + a_{3,2,2} ~\leq~ 1$
    \end{description}
\end{itemize}

\bigskip

\noindent
\underline{\textsf{A solution:}} One solution that satisfies
all the above constraints is obtained by setting $a_{2,1,1}$, $a_{3,2,1}$, 
$a_{1,1,2}$ and $a_{3,2,2}$ to 1 and all the other variables to 0.
This leads to the following matching in two rounds.
In Round 1, $x_2$ and $x_3$ are matched to $y_1$ and $y_2$
respectively; in Round 2, $x_1$ and $x_3$ are matched 
to $y_1$ and $y_2$ respectively.

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Information for Section~\ref{sec:min_round_req_one}}

\medskip

\subsection{An Example to Illustrate the Construction in
Figure~\ref{fig:alg_problemrone}}

\begin{figure}[h]
\rule{\columnwidth}{0.01in}
\begin{minipage}{0.45\columnwidth}
%\smallskip
\centering
\input{graph_one.pdf_t}
\end{minipage}
\quad
%\hspace*{0.1in}
\begin{minipage}{0.45\columnwidth}
%\smallskip
\centering
\input{graph_two.pdf_t}
\end{minipage}
\caption{An example to illustrate the algorithm in Figure~\ref{fig:alg_problemrone}.
The graph on the left is the original compatibility graph.
The graph on the right is the new graph produced by the Algorithm
in Step~1 with $k = 2$.
(The new edges are shown as dashes.)
The graph on the left has a two round matching $M_1$, $M_2$ that 
matches each agent once: $M_1 = \{(x_1, y_1), (x_2, y_2)\}$ and
$M_2 = \{(x_3, y_1)\}$.
The corresponding maximum matching in the graph on the right
is $\bbm' ~=~ \{(x_1, y_{1,1}), (x_2, y_{2,1}), (x_3, y_{1,2})\}$.
}
\label{fig:example_alg_problemrone}
\rule{\columnwidth}{0.01in}
\end{figure}

\bigskip

\subsection{Statement and Proof of Lemma~\ref{lem:alg_problemrone}}

\medskip

\noindent
\textbf{Statement of Lemma~\ref{lem:alg_problemrone}:}~
Algorithm \algproblemrone{} (a) produces a solution iff the compatibility
graph \comgr{} has a $k$-round matching such that each 
agent appears in one of the $k$ matchings, and 
(b) runs in polynomial time. 



\smallskip

\noindent
\textbf{Proof:} 
\textbf{Part (a):}~\textsf{If part:} Suppose \comgr{} contains a $k$-round matching
$M_1$, $M_2$, $\ldots$, $M_k$ such that each agent $x_i$ appears
in one of the $k$ matchings.
We may assume without loss of generality that each
agent $x_i$ appears in exactly one matching.
(If an agent occurs in two or more matchings, we can remove all
but one of the occurrences.)
We will show that $G'$ has a matching that contains each node of \agset.
To see this,
consider the following set $\bbm'$ of edges in $G'$: for each edge
$(x_i, y_j)$ that appears in matching $M_p$ for some $p$ 
($1 \leq p \leq k$), add the edge
$(x_i, y_{j,p})$ to $\bbm'$.
Since each agent $x_i$ appears in one of the $k$ matchings  
of \comgr, the agent also appears in one of the edges in $\bbm'$.
To show that $\bbm'$ is a matching, we will show by contradiction
that no node in \bbr{} appears in two or more edges of $\bbm'$.
So, assume that some node $y_{j,p}$ appears in two edges, say
$(x_a, y_{j,p})$ and $(x_b, y_{j,p})$, of $\bbm'$.
By our construction of $\bbm'$, this happened because matching $M_p$
contains both the edges $(x_a, y_j)$ and $(x_b, y_j)$.
This contradicts the assumption that $M_p$ is a matching and
shows that $\bbm'$ is a matching that contains all the agents. 

\smallskip

\noindent
\textsf{Only If part:} Suppose $G'$ contains
a matching $\bbm'$ that includes all the agents.
We need to show that there is a set of at most $k$ matchings
$M_1$, $M_2$, $\ldots$, $M_k$ of \comgr{} such that
each agent appears in one of these matchings.
This can be done as follows.
Initially, each $M_p$ is empty, $1 \leq p \leq k$.
For each edge $(x_i, y_{j,p})$ in $\bbm'$, add the edge $(x_i, y_j)$ 
to $M_p$.
Since $\bbm'$ contains each agent $x_i$ once, by our construction,
$x_i$ appears as an end point of just one edge 
in some set $M_p$.
We will show by contradiction that each nonempty $M_p$ is a matching
in \comgr.
So, suppose for some $p$, $M_p$ is not a matching.
Since each $x_i$ appears in just one edge of $\bbm'$, 
if $M_p$ is not a matching, then some node $y_j$ appears
in two edges $(x_a, y_j)$ and $(x_b, y_j)$ in $M_p$.
By our construction, this happened because the edges $(x_a, y_{j,p})$
and $(x_b, y_{j,p})$ appear in $\bbm'$.
This contradicts the assumption that $\bbm'$ is matching in $G'$.
This completes our proof of the Only If part and also that of
Part~(a) of Lemma~\ref{lem:alg_problemrone}.

\smallskip

\noindent
\textbf{Part (b):}~ We now consider the running time of
\algproblemrone{}.
Step~1 which constructs the graph $G'$
can be carried out in time $O(n + km + k|E|)$ time. 
Step~2 finds a maximum matching in $G'$.
Since $G'$ has $n + km$ nodes and $k|E|$ edges,
a maximum matching in $G'$ can be found in 
$O(k|E|\,\sqrt{n + km})$
time using well known algorithms for maximum matching \cite{Hopcroft-Karp-1973}.
Since the matching $\bbm'$ has $n$ edges (i.e., exactly one
edge per agent), we can find the corresponding $k$ matchings of $G$
in $O(n)$ time.
Thus, the running time of the algorithm is dominated by Step~2.
In other words, the running time of the algorithm is 
$O(k|E|\,\sqrt{n + km})$. \QED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
\iffalse
%%%%%%%%%%%%%%%%%%%%%
To prove the approximation result, we note that for a universe $U$
with $t$ elements, the MSC problem cannot be approximated to within
the factor $o(\log{t})$ in polynomial time, unless \textbf{P} = \cnp{}
\cite{Vaz-2001}.
The above construction produces an instance of \agmrm{}{}{} such that
if the number of rounds must beat most $t$,
for any solution to MSC of cost $\alpha$ corresponds to a solution
for the \agmrm{} instance where the
budget of agent $x^*$ is equal to $\alpha$ and vice versa.
(In other words, when the number of rounds must be at most $t$,
the above reduction from MSC to \agmrm{} is approximation
preserving.)
Thus, the approximation hardness of \agmrm{} directly follows from that
of MSC.  \qed
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%%%%%
To prove the approximation result, we note that for a universe $U$
with $t$ elements, the MSC problem cannot be approximated to within
the factor $o(\log{t})$ in polynomial time, unless \textbf{P} = \cnp{}
\cite{Vaz-2001}.
The above construction produces an instance of \agmrm{}{}{} such that
if the number of rounds must beat most $t$,
for any solution to MSC of cost $\alpha$ corresponds to a solution
for the \agmrm{} instance where the
budget of agent $x^*$ is equal to $\alpha$ and vice versa.
(In other words, when the number of rounds must be at most $t$,
the above reduction from MSC to \agmrm{} is approximation
preserving.)
Thus, the approximation hardness of \agmrm{} directly follows from that
of MSC.  \qed
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Information for Section~\ref{sec:min_round_req_one}}

\medskip

\subsection{An Example to Illustrate the Construction in
Figure~\ref{fig:alg_problemrone}}

\begin{figure}[h]
\rule{\columnwidth}{0.01in}
\begin{minipage}{0.45\columnwidth}
%\smallskip
\centering
\input{graph_one.pdf_t}
\end{minipage}
\quad
%\hspace*{0.1in}
\begin{minipage}{0.45\columnwidth}
%\smallskip
\centering
\input{graph_two.pdf_t}
\end{minipage}
\caption{An example to illustrate the algorithm in Figure~\ref{fig:alg_problemrone}.
The graph on the left is the original compatibility graph.
The graph on the right is the new graph produced by the Algorithm
in Step~1 with $k = 2$.
(The new edges are shown as dashes.)
The graph on the left has a two round matching $M_1$, $M_2$ that 
matches each agent once: $M_1 = \{(x_1, y_1), (x_2, y_2)\}$ and
$M_2 = \{(x_3, y_1)\}$.
The corresponding maximum matching in the graph on the right
is $\bbm' ~=~ \{(x_1, y_{1,1}), (x_2, y_{2,1}), (x_3, y_{1,2})\}$.
}
\label{fig:example_alg_problemrone}
\rule{\columnwidth}{0.01in}
\end{figure}

\bigskip

\subsection{Statement and Proof of Lemma~\ref{lem:alg_problemrone}}

\medskip

\noindent
\textbf{Statement of Lemma~\ref{lem:alg_problemrone}:}~
Algorithm \algproblemrone{} (a) produces a solution iff the compatibility
graph \comgr{} has a $k$-round matching such that each 
agent appears in one of the $k$ matchings, and 
(b) runs in polynomial time. 



\smallskip

\noindent
\textbf{Proof:} 
\textbf{Part (a):}~\textsf{If part:} Suppose \comgr{} contains a $k$-round matching
$M_1$, $M_2$, $\ldots$, $M_k$ such that each agent $x_i$ appears
in one of the $k$ matchings.
We may assume without loss of generality that each
agent $x_i$ appears in exactly one matching.
(If an agent occurs in two or more matchings, we can remove all
but one of the occurrences.)
We will show that $G'$ has a matching that contains each node of \agset.
To see this,
consider the following set $\bbm'$ of edges in $G'$: for each edge
$(x_i, y_j)$ that appears in matching $M_p$ for some $p$ 
($1 \leq p \leq k$), add the edge
$(x_i, y_{j,p})$ to $\bbm'$.
Since each agent $x_i$ appears in one of the $k$ matchings  
of \comgr, the agent also appears in one of the edges in $\bbm'$.
To show that $\bbm'$ is a matching, we will show by contradiction
that no node in \bbr{} appears in two or more edges of $\bbm'$.
So, assume that some node $y_{j,p}$ appears in two edges, say
$(x_a, y_{j,p})$ and $(x_b, y_{j,p})$, of $\bbm'$.
By our construction of $\bbm'$, this happened because matching $M_p$
contains both the edges $(x_a, y_j)$ and $(x_b, y_j)$.
This contradicts the assumption that $M_p$ is a matching and
shows that $\bbm'$ is a matching that contains all the agents. 

\smallskip

\noindent
\textsf{Only If part:} Suppose $G'$ contains
a matching $\bbm'$ that includes all the agents.
We need to show that there is a set of at most $k$ matchings
$M_1$, $M_2$, $\ldots$, $M_k$ of \comgr{} such that
each agent appears in one of these matchings.
This can be done as follows.
Initially, each $M_p$ is empty, $1 \leq p \leq k$.
For each edge $(x_i, y_{j,p})$ in $\bbm'$, add the edge $(x_i, y_j)$ 
to $M_p$.
Since $\bbm'$ contains each agent $x_i$ once, by our construction,
$x_i$ appears as an end point of just one edge 
in some set $M_p$.
We will show by contradiction that each nonempty $M_p$ is a matching
in \comgr.
So, suppose for some $p$, $M_p$ is not a matching.
Since each $x_i$ appears in just one edge of $\bbm'$, 
if $M_p$ is not a matching, then some node $y_j$ appears
in two edges $(x_a, y_j)$ and $(x_b, y_j)$ in $M_p$.
By our construction, this happened because the edges $(x_a, y_{j,p})$
and $(x_b, y_{j,p})$ appear in $\bbm'$.
This contradicts the assumption that $\bbm'$ is matching in $G'$.
This completes our proof of the Only If part and also that of
Part~(a) of Lemma~\ref{lem:alg_problemrone}.

\smallskip

\noindent
\textbf{Part (b):}~ We now consider the running time of
\algproblemrone{}.
Step~1 which constructs the graph $G'$
can be carried out in time $O(n + km + k|E|)$ time. 
Step~2 finds a maximum matching in $G'$.
Since $G'$ has $n + km$ nodes and $k|E|$ edges,
a maximum matching in $G'$ can be found in 
$O(k|E|\,\sqrt{n + km})$
time using well known algorithms for maximum matching \cite{Hopcroft-Karp-1973}.
Since the matching $\bbm'$ has $n$ edges (i.e., exactly one
edge per agent), we can find the corresponding $k$ matchings of $G$
in $O(n)$ time.
Thus, the running time of the algorithm is dominated by Step~2.
In other words, the running time of the algorithm is 
$O(k|E|\,\sqrt{n + km})$. \QED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\bigskip

\section{Additional Material for Section~\ref{sec:mrm_poly}}

\medskip

The steps of our algorithm \algmrm{} for \mrm{} were
shown in Figure~\ref{fig:alg-mrma-prb}.
A slightly more detailed version of the algorithm that
mentions the intuition behind some of the steps
appears in Figure~\ref{fig:detailed-alg-mrma-prb}.

\begin{figure}[ht]
\rule{\columnwidth}{0.01in}
%\noindent
%textbf{Steps of the Algorithm:}

\begin{enumerate}
\item Starting from the given compatibility graph $G(X, Y, E)$,
create a new bipartite graph $G'(V', W', E')$ as follows.
To begin with, the sets  $V'$, $W'$ and $E'$ are all empty.
   \begin{enumerate}
      \item For each resource node $y_j \in Y$, add $k$ nodes denoted
      by $y_j^t$, where $t = 1, 2, \ldots, k$, to $W'$.
      (\textbf{Intuition:}~ If node $y_j^t$ is included in the
       matching, the interpretation is that resource $y_j \in Y$ is
       matched to some agent in round $t$.)

      \item For each agent node $x_i \in X$ with requirement $\rho_i = 1$,
      do the following.
         \begin{enumerate}
            \item Add a new node $x_i^1$ to $V'$.
            \item For each edge $\{x_i, y_j\} \in E$, do the following:
            for each $t \in K_i$, add the edge $\{x_i^1, y_j^t\}$
            to $E'$.
         \end{enumerate}

      \item For each agent node $x_i \in X$ with requirement $\rho_i \geq 2$,
      do the following.
         \begin{enumerate}
            \item For each $t \in K_i$, add a node denoted by $x_i^t$ to $V'$.
            (\textbf{Intuition:}~ If node $x_i^t$ is included in the
             matching, the interpretation is that agent $x_i$ is matched
             to some resource in round $t$.)
           \item Add $q_i = |K_i|- \rho_i$ ``dummy-resource" nodes, denoted
            by $z_i^{\ell}$, where $\ell = 1, 2, \ldots, q_i$, to $W'$.
            (\textbf{Intuition:} Matching an agent node $x_i^t$ to a
             dummy-resource node
             $z_i^{\ell}$ means that agent $x_i$ is \emph{not} matched
             in round $t$.)

            \item For each edge $\{x_i, y_j\} \in E$ and each $t \in K_i$,
             add the edge $\{x_i^t, y_j^t\}$ to $E'$.

            \item For each node $x_i^t$, add the
            $|K_i|- \rho_i$ edges $\{x_i^t, z_i^{\ell}\}$,
            $1 \leq \ell \leq |K_i|-\rho_i$, to $E'$.
         \end{enumerate}
   \end{enumerate}
\item Find a maximum matching $M'$ in $G'(V', W', E')$.

\item If $M'$ does \emph{not} include all the nodes in $V'$, then
      print ``No Solution" and \textbf{stop}.

\item Otherwise (i.e., $M'$ includes all the nodes in $V'$),
compute a collection of matchings $M_1$, $M_2$, $\ldots$, $M_k$, for
$G$ as follows. (\textbf{Note:}~ At the end, some of these matchings
may be empty.)
    \begin{enumerate}
      \item For each $\ell$, $1 \leq \ell \leq k$, initialize
      $M_{\ell}$ to the empty set.
      \item For each edge $e \in M'$ that does \emph{not} use a
      dummy resource, do the following.
             \begin{enumerate}
                \item Let $x_i^{t}$ and $y_j^{\ell}$ denote the
                      end points of $e$.
                \item Add the edge $\{x_i, y_j\}$ to $M_{\ell}$.
              \end{enumerate}
       \end{enumerate}
\end{enumerate}
\caption{A More Detailed Description of the Steps of \algmrm{} for \mrm{}}
\label{fig:detailed-alg-mrma-prb}
\rule{\columnwidth}{0.01in}
\end{figure}      
An example to illustrate the construction used in Step~1 of
the algorithm is shown in Figure~\ref{fig:constr_example}.
In that example, the compatibility graph $G(X, Y, E)$ (shown in
the left panel of Figure~\ref{fig:constr_example})  has three agent nodes
($x_1$, $x_2$, $x_3$) and two resource nodes ($y_1$ and $y_2$).
The number of rounds ($k$) is 3.
For each agent $x_i$, the set of allowed rounds 
$K_i = \{1, 2, 3\}$, $1 \leq i \leq 3$.
The requirements for agents
$x_1$, $x_2$ and $x_3$ are 1, 2 and 2 respectively. 
The right panel of Figure~\ref{fig:constr_example} shows
the new graph $G'(V', E', W')$ generated at the end of Step~1
of the Algorithm in Figure~\ref{fig:alg-mrma-prb}.
A maximum matching (of size 7) in the graph $G'$ and
the corresponding 3-round solution to the \mrm{}
for the graph $G$ are shown in Figure~\ref{fig:sol-mmra-prb}.

\begin{figure}[tb]
\noindent
\rule{\columnwidth}{0.01in}
\smallskip

\centering
\input{ex_compatibility_graph.pdf_t}
\caption{An Example to Illustrate the Construction Used in
the Algorithm of Figure~\ref{fig:alg-mrma-prb}.
The left panel shows the original compatibility graph $G(X, Y, E)$
where the requirements $\rho_1$, $\rho_2$ and $\rho_3$
for agent nodes $x_1$, $x_2$ and $x_3$ are 1, 2 and 2 respectively.
The number of rounds $k$ is set to 3.
The right panel shows the new graph $G(V', W', E')$ constructed
using the the Algorithm of Figure~\ref{fig:alg-mrma-prb}.
The dummy resource nodes ($z_2^1$ and $z_3^1$) are shown as
open rectangles.}
\label{fig:constr_example}
\smallskip
\noindent
\rule{\columnwidth}{0.01in}
\end{figure}

\begin{figure}[htb]
\rule{\columnwidth}{0.01in}
\begin{minipage}{0.55\columnwidth}
\smallskip
\centering
\input{matching_larger_graph.pdf_t}
\smallskip
\end{minipage}
\hspace*{0.1in}
\begin{minipage}{0.35\columnwidth}
\textbf{Three-Round Solution for $G$:}
\begin{eqnarray*}
M_1 & = & \{\{x_1, y_1\}, \{x_2, y_2\}\} \\ 
M_2 & = & \{\{x_2, y_1\}, \{x_3, y_2\}\} \\ 
M_3 & = & \{\{x_3, y_2\}\} \\ 
\end{eqnarray*}
%\smallskip
\end{minipage}
\caption{A Maximum Matching for $G'$ and the
corresponding Three-Round Solution for $G$}
\label{fig:sol-mmra-prb}
\smallskip
\noindent
\rule{\columnwidth}{0.01in}
\end{figure}

\medskip

\noindent
\textbf{Statement and Proof of Theorem~\ref{thm:alg_mmra_prb_correct}:}
(i) There is a solution to the \mrm{} instance iff the graph
$G'$ constructed in Step~1 of Algorithm
\algmrm{} has a matching of size $|V'|$.
(ii) The running time of the lgorithm is
$O(k^{3/2}|E| \sqrt{|X|+|Y|})$.

\smallskip

\noindent
\textbf{Proof:}

\smallskip

\noindent
\textbf{Part (i):}~
Suppose $G'$ has a matching $M'$ of size $|V'|$.
Thus, $M'$ includes every node in $V'$.
We will show that the solution produced in Step~4 of \algmrm{}
satisfies the requirements of each agent by
considering two cases.

\smallskip

\noindent
\underline{Case 1:}~ Agent $x_i$ has requirement $\rho_i = 1$.
The node corresponding to $x_i$ in $G'$
is $x_i^1$. Note that $x_i^1$ is not adjacent to any dummy resource
node in $W'$.
Further, each edge adjacent to $x_i^1$ is of the form $\{x_I^1, y_j^t\}$
for some $t \in K_i$.
Thus, $M'$ must have the edge $\{x_i^1, y_j^t\}$
for some $j$ and some $t \in K_i$.
Since $M'$ is a matching, no other edge in $M'$
is incident on $y_j^t$. In our solution, the edge $\{x_i, y_j\}$
is added to $M_t$; that is, agent $x_i$ is matched to resource $y_j$
in round $t$.

\smallskip

\noindent
\underline{Case 2:}~ Agent $x_i$ has requirement $\rho_i \geq 2$.
Let $S_i = \{x_i^{\ell}: 1 \leq \ell \leq |K_i|\}$
denote the set of $|K_i|$ nodes in $G'$ that correspond to $x_i$.
Since only $|K_i|-\rho_i$ dummy resource nodes corresponding
to $x_i$ were added to $G'$, at least $\rho_i$ nodes in $S_i$
must be matched in $M'$ to non-dummy resource nodes.
Let $S'_i \subseteq S_i$ denote the subset of nodes of $S_i$
that are matched in $M'$ to non-dummy resource nodes.
Further, each $x_i^{\ell}$ has edges only to nodes of the form $y_j^{\ell}$.
Thus, for each node $x_i^{\ell} \in S'_i$, $M'$ contains the
edge $\{x_i^{\ell}, y_j^{\ell}\}$ for some $j$.
In other words, by considering $S'_i$, we can
find at least $\rho_i$ rounds and the corresponding resources
with which $x_i$ is matched in $\rho_i$  of the rounds in $K_i$.

We thus have a solution to the \mrm{} instance.

\medskip

For the converse, suppose there is a solution to the \mrm{}
instance consisting of $k$ matchings
given by $M_1$, $M_2$, $\ldots$, $M_k$.
By deleting edges from these matching arbitrarily, we can
ensure that each node $x_i$ with requirement $\rho_i$ appears
in exactly $\rho_i$ of the matchings $M_1$, $M_2$, $\ldots$, $M_k$.
We refer to this as the \textbf{pruning step} in the following discussion.
For simplicity, let the the matchings after the pruning step
be also denoted by $M_1$, $M_2$, $\ldots$, $M_k$.
We construct a matching $M'$ of size $|V'|$ for $G'(V', W', E')$
as follows.
Initially, $M'$ is empty.
\begin{enumerate}
\item Consider each node $x_i$ of $G$ such that $\rho_i = 1$.
By our pruning step, $x_i$ appears in just one matching,
say $M_t$, for some $t \in K_i$. Let $M_t$ contain the edge $\{x_i, y_j\}$.
By our construction of $G'$, the edge $\{x_i^1, y_j^t\}$ is in $E'$,
and we add that edge to $M'$.

\item Consider each node $x_i$ of $G$ such that $\rho_i \geq 2$.
By our pruning step, $x_i$ appears in exactly $\rho_i$ of the matchings
$M_1$, $M_2$, $\ldots$, $M_k$.
Let $H = \{1, 2, \ldots, k\}$.
Further, let $H_i = \{p_1, p_2, \ldots, p_{\rho_i}\}$ $\subseteq$ $H$
denote the set of indices such that for each $p_{\ell} \in H_i$,
$x_i$ appears in the matching $M_{p_{\ell}}$.
Note that $H_i \subseteq K_i$ and $|H_i| = \rho_i$.
By our construction of $G'$, for each $p_{\ell} \in H_i$,
the edge $\{x_i^{p_{\ell}}, y_j^{p_{\ell}}\}$ is in $E'$,
for some $j$.
For each $p_{\ell} \in H_i$, we
add the edge $\{x_i^{p_{\ell}}, y_j^{p_{\ell}}\}$ to $M'$.
Further, for $x_i$, $W'$ has a set $Z_i =$
$\{z_i^1, z_i^2, \ldots, z_i^{q_i}\}$ with $q_i = |K_i|-\rho_i$
dummy resource nodes.
For each node $x_i^t \in V'$ such that $t \not\in H_i$, we can match
$x_i^t$ with an arbitrary node in $Z_i$ and add the corresponding
edge to $M'$.
This ensures that $M'$ includes all the $|K_i|$ nodes in $V'$ that
correspond to $x_i$.
\end{enumerate}
Thus, the resulting $M'$ includes every node in $V'$.
This completes our proof of Part~(i).

\medskip

\noindent
\textbf{Part (ii):}~ We first estimate the number of nodes and
edges in $G'$.
For each node in $X \cup Y$ of $G'$, $G'$ adds at most $k$
nodes to $G'$.
Further, for each node in $X$, $G'$ has at most $k$ dummy
resource nodes.
Therefore, the total number of nodes in $G'$ is at most
$(k+1)|X| + k|Y|$ = $O(k(|X|+|Y|))$.
For each edge in $E$, at most $k$ edges are added to $G'$.
Further, for each node in $X$, at most $k$ edges are added to
dummy resource nodes of $G'$.
Therefore, the total number of edges in $G'$ is at most
$k|E| + k|X|$.
Since each agent is compatible with at least one resource,
we have $|X| \geq |E|$.
Thus, the number of edges in $G'$ = $O(k|E|)$.
In other words, Step~1 runs in $O(k(|X| + |Y| + |E|))$ time.
For any bipartite graph $\calh(V_{\mathcal{H}}, W_{\mathcal{H}}, 
E_{\mathcal{H}})$,
it is well known that a maximum matching can be computed in
time $O(|E_{\mathcal{H}}| \times \sqrt{|V_{\mathcal{H}} 
+ |W_{\mathcal{H}}|})$ \cite{CLRS-2009}.
Thus, the running time of Step~2 is
$O(k|E| \sqrt{k(|X|+|Y|)})$ =
$O(k^{3/2}|E| \sqrt{|X|+|Y|})$.
The matching $M'$ is of size $O(k|X|)$ and Step~4 of
the algorithm uses $O(1)$ time per edge in $M'$ to construct
the $k$-round matchings. Thus, Step~4 runs in $O(k|X|)$ time.
Thus, the dominant part of the running time is due to Step~2.
In other words, the running time of Algorithm~\algmrm{} is
$O(k^{3/2}|E| \sqrt{|X|+|Y|})$. \hfill$\Box$

\section{Additional Material for Section~\ref{sec:algmaxagmrm}}

\medskip

\begin{table}[htbp]
\begin{center}
\begin{tabular}{|c|p{4.5in}|}\hline
\textbf{Symbol} & \textbf{Explanation}\\ \hline\hline
\agset{} & Set of $n$ agents; \agset{} = $\{x_1, x_2, \ldots, x_n\}$ \\ \hline
\rset{} & Set of $m$ resources; \rset{} = $\{y_1, y_2, \ldots, y_m\}$ \\ \hline
$\calc_i$ & Set of labels $\{c_i^1, c_i^2, \ldots, c_i^{\ell_i}\}$
            of associated with agent $x_i$, $1 \leq i \leq n$.
            (Thus, $\ell_i = |\calc_i|$.)
            \\ \hline
$\psi_i^t$ & Cost of removing the label $c_i^t$, $1 \leq t \leq \ell_i$ and
               $1 \leq i \leq n$.  \\ \hline
$\beta_i$ & Cost budget for agent $x_i$, $1 \leq i \leq n$.
            (This is the total cost agent $x_i$ may spend
             on removing labels.)
            \\ \hline
$\rho_i$  & The minimum number of times an agent must appear in the
            set of matchings. \\ \hline
$\Gamma_e$ & Set of labels appearing on edge $e$. (If an edge $e$ joins
             agent $x_i$ to resource $y_j$, then $\Gamma_e \subseteq \calc_i$.)
             Edge $e$ can be added to the compatibility graph only
             after \emph{all} the labels in $\Gamma_e$ are removed.
            \\ \hline
$k$ & Upper bound on the number of rounds of matching \\ \hline
\end{tabular}
\end{center}
\caption{Notation Used in the Definition of \agmrm{}{}{}{}
and the ILP Formulation of Section~\ref{sec:general_ilp}}
\label{tab:notation}
\end{table}





%%%%%%%%%%%%%% From here on, all the material in this file %%%%%%%%
%%%%%%%%%%%%%% has been commented out.                  %%%%%%%%%%%
\iffalse

%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Material for 
Section~\ref{sec:methods_per_round_budget}}

\medskip

\subsection{A Simpler ILP for \maxmrm{}}
\label{sup:sse:simpler_ilp}

Section~\ref{sec:general_ilp} presented an ILP for \maxagmrm{}.
Here, we present a simpler ILP for \maxmrm{} where 
the compatibility graph $G(X, Y, E)$ is given.

\smallskip

\noindent
\textbf{ILP Formulation:}~ 

\smallskip

\noindent
\underline{\textsf{Variables:}} 
\begin{itemize}
\item For each agent $x_i$, let $A_i$ denote the
set of resources with which $x_i$ is compatible;
that is, $A_i = \{y_j ~:~ \{x_i, y_j\} \in E\}$, $1 \leq i \leq n$.
For each agent $x_i$ and each resource $y_j \in A_i$,
we have $k$ \{0,1\}-variables
denoted by $a_{ijr}$, where $1 \leq i \leq n$, $1 \leq j \leq m$ and
$1 \leq r \leq k$.
The interpretation is that  $a_{ijr}$ is 1 iff agent $x_i$ is matched
to resource $y_j$ in round $r$.

\item For each agent $x_i$, we have a non-negative integer
variable $\eta_i$ which gives the number of rounds
in which $x_i$ is matched.

\item For each agent $x_i$, we have a \{0,1\}-variable $s_i$
that is 1 iff agent $x_i$'s requirement is satisfied.
\end{itemize}

\smallskip

\noindent
\underline{\textsf{Objective:}}~ Maximize~~
$\sum_{i=1}^{n} s_i$.

\smallskip

\noindent
\underline{\textsf{Constraints:}} 

\begin{itemize} [leftmargin=*,noitemsep,topsep=0pt]
\item For each agent $x_i$, the number of rounds
in which $x_i$ is matched should equal $\eta_i$.
This constraint can be expressed as
\begin{equation}
\sum_{r=1}^{k}\: \sum_{y_j \in A_i} a_{ijr} ~=~ \eta_i, ~~1 \leq i \leq n
%\label{eqn:v1_agent_deg}
\end{equation}

\item Each agent $x_i$ is matched to a resource \emph{at most once}
in each round.  This constraint can be expressed as
\begin{equation}
\sum_{y_j \in A_i}\: a_{ijr} ~\leq~ 1, ~~1 \leq i \leq n,~~ 1 \leq r \leq k
\end{equation}

\item For each resource $y_j$, let $B_j$ denote the set of agents
with which $y_j$ is compatible, $1 \leq j \leq m$;
that is, $B_j = \{x_i ~:~ \{x_i, y_j\} \in E\}$, $1 \leq j \leq m$.
In each round, each resource must be matched to an agent
\emph{at most} once. 
This constraint can be expressed as
\begin{equation}
\sum_{x_i \in B_j} a_{ijr} ~\leq~ 1, ~~
               1 \leq j \leq m,~~ 1 \leq r \leq k 
%\label{eqn:v1_res_deg}
\end{equation}

\item The rounds in which an agent $x_i$ is matched
must be in $K_i$. The corresponding constraint is:
\begin{align}
    a_{ijr} ~=~ 0, ~~ r \not\in K_i,~ 1 \leq j \leq m,~
     1 \leq i \leq n
\end{align}

\item Variable $s_i$ to be 1
iff agent $x_i$ was matched
in at least $\rho_i$ rounds. The following constraints,
which must hold for each $i$, $1 \leq i \leq n$, ensure this
condition.
\begin{eqnarray*}
k\,s_i ~\leq~ \eta_i - \rho_i + k \\
k\,s_i ~\geq~ \eta_i - \rho_i + 1 
\end{eqnarray*}

\item $a_{ijr} \in \{0,1\}$, 
$1 \leq i \leq n$,~ $1 \leq j \leq m$,~ $1 \leq r \leq k$.
\end{itemize}

\medskip

\noindent
\underline{\textsf{Obtaining a Solution:}} After solving
the ILP, for each variable $a_{ijr}$ which is set to 1 in the
solution, we match agent $x_i$ with resource $y_j$ in round $r$.
%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%\input{ilp_many_requirement_matching}

\iffalse
%%%%%%%%%%%%%%%%%%%%%%
\medskip
We now present an example to illustrate the above ILP
formulation.

\noindent
\textbf{Example:} In the compatibility graph shown below,
we have an agent $x_3$ which must appear in at least two rounds
of matching. 
(Recall from Section~\ref{sec:general_ilp} that for each agent
$x_i$, $A_i$ is the set of resources to which $x_i$
can be matched. Likewise, for each resource
$y_j$, $B_j$ is the set of agents to which $y_j$
can be matched.)

\bigskip

\begin{center}
\begin{minipage}{0.3\textwidth}
\input{graph_one.pdf_t}
\end{minipage}
\hspace*{0.1in}
\begin{minipage}{0.4\textwidth}
\begin{itemize}
\item Let $k = 2$.
\item Let $\rho_1 = 1$, $\rho_2 = 1$ and $\rho_3 = 2$.
\item $A_1 = \{y_1\}$, $A_2 = A_3 = \{y_1, y_2\}$.
\item $B_1 = \{x_1, x_2, x_3\}$ and $B_2 = \{x_2, x_3\}$.
\end{itemize}
\end{minipage}
\end{center}

\medskip

\noindent
The ILP for the above problem instance is as follows.

\bigskip

\noindent
\underline{\textsf{Variables:}}~ 
$a_{1,1,1}$, $a_{1,1,2}$,
$a_{2,1,1}$, $a_{2,1,2}$,
$a_{2,2,1}$, $a_{2,2,2}$,
$a_{3,1,1}$, $a_{3,1,2}$,
$a_{3,2,1}$ and $a_{3,2,2}$.
(Each of these variables takes on a value from $\{0,1\}$.
The significance of variable $a_{ijr}$ is that it takes on the
value 1 iff agent $x_i$ is assigned resource $y_j$ in round $r$.)

\bigskip

\noindent
\underline{\textsf{Constraints:}} 

\begin{itemize}
\item For Agent $x_1$: (i) $a_{1,1,1} + a_{1,1,2} ~\geq~ 1$,~
(ii) $a_{1,1,1} \leq 1$~ and (iii) $a_{1,1,2} \leq 1$. 
(The last two constraints can be omitted since the fact
that each variable takes on a value from $\{0,1\}$
implies each of the last two constraints.)

\item For Agent $x_2$: (i) $a_{2,1,1} + a_{2,2,1} 
                        +a_{2,1,2} + a_{2,2,2} ~\geq~ 1$,~
                (ii) $a_{2,1,1} + a_{2,2,1} ~\leq~ 1$~ and 
                (iii) $a_{2,1,2} + a_{2,2,2} ~\leq~ 1$.

\item For Agent $x_3$: (i) $a_{3,1,1} + a_{3,2,1} 
                        +a_{3,1,2} + a_{3,2,2} ~\geq~ 2$,~
                       (ii) $a_{3,1,1} + a_{3,2,1} ~\leq~ 1$ and
                       (iii) $a_{3,1,2} + a_{3,2,2} ~\leq~ 2$.

\item For Resource $y_1$: 
    \begin{description}
      \item{(a)} $a_{1,1,1} + a_{2,1,1} + a_{3,1,1} ~\leq~ 1$
      \item{(b)} $a_{1,1,2} + a_{2,1,2} + a_{3,1,2} ~\leq~ 1$
    \end{description}

\item For Resource $y_2$: 
    \begin{description}
      \item{(a)} $a_{2,2,1} + a_{3,2,1} ~\leq~ 1$
      \item{(b)} $a_{2,2,2} + a_{3,2,2} ~\leq~ 1$
    \end{description}
\end{itemize}

\bigskip

\noindent
\underline{\textsf{A solution:}} One solution that satisfies
all the above constraints is obtained by setting $a_{2,1,1}$, $a_{3,2,1}$, 
$a_{1,1,2}$ and $a_{3,2,2}$ to 1 and all the other variables to 0.
This leads to the following matching in two rounds.
In Round 1, $x_2$ and $x_3$ are matched to $y_1$ and $y_2$
respectively; in Round 2, $x_1$ and $x_3$ are matched 
to $y_1$ and $y_2$ respectively.

\section{Additional Material for Section~\ref{sec:experiments}}
\label{sup:sec:experiments}
Due to space limitation, we could not include the results of our experiments
with the \pv{} dataset in the context of \problemrone{} (\agmrm{} with
requirement at least one) in the main paper. Those results are in
Figure~\ref{mrmar1_pv}. The experiment design is same as that explained
for Figure~\ref{mrmar1} (first three plots) with regard to \cc{}
experiments. We note that the results indicate that among all
restrictions, activity preferences of children is the one that leads to the
most reduction in the number of rounds required when relaxed. Also, we note
that, unlike in the \cc{} case, relaxation of combinations of attributes
does not have much effect compared to relaxation of the activity preference
alone..
%%
\begin{figure}[!htb]
    \centering
    \includegraphics[width=.32\columnwidth]{figures/mrmar1_pv_1.pdf}
    \includegraphics[width=.32\columnwidth]{figures/mrmar1_pv_2.pdf}
    \includegraphics[width=.32\columnwidth]{figures/mrmar1_pv_3.pdf}
    \caption{\problemrone{} results for \pv{}. In
the \pv{} plots, for relaxations beyond the values on the $x$-axes,
the results are unchanged.}
\label{mrmar1_pv}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.5\columnwidth]{figures/mrma_heuristic_pv.pdf}
    \caption{\SAproblem{} results for \pv{}. The graph that compares \SAproblem{} to \ilpproblem{} is not presented since the runtime of  \ilpproblem{} on the \pv{} dataset is too long and not practical. }
\label{mrmar1_pv_2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%, receives a restrictions graph and a budget $\beta_i$ for each  agent. It generates compatibility graphs that are 
%possible given the budgets.
%To evaluate the compatibility graphs, \SAproblem{} uses 
%\greedyproblemprb{} that returns the minimum number of rounds that are needed, given agents' requirements.
%In the first step, it randomly generates a set of relaxations for each agent; these relaxations satisfy the budget constraints and are Pareto Optimal (PO). It then obtains the minimum number %of rounds $k$ using \greedyproblemprb{} for the resulting compatible graph as the value for the local search based on Simulated Annealing  In the next step, it randomly chooses one of the %agents and generates a new random relaxation for this agent that again satisfies the budget and is PO. For the new compatibility graph, it obtains $k'$ using \greedyproblemprb. If $k' \leq %k$, it adopts the new relaxations. Otherwise, it uses the Simulated Annealing approach to make the decision  and in both cases, if time permits, it continues its search. 

%% \begin{figure}[htbp]
%% \rule{\columnwidth}{0.01in}
%% %\textbf{Steps of Heuristic}
%% \begin{enumerate}
%% \item	Let $G=(X,Y,E)$ be the compatibility graph.
%% \item	$\forall x\in X$, $\rho_x$  is the no. of required matchings for agent $x$.
%% \item	$k_1 \leftarrow$  Minimum $k$ such that there exist $k$ matchings for which each node participates in at least one.
%% %\item	$mx=\max_{T}(x\in X)⁡(r_x )$%SSR corrected this.
%% \item	$mx=\max_{x\in X}\,(\rho_x)$
%% 	\item $\forall x \in X$, $e_x \leftarrow 0$. ($e_x$ is the no. of times agent $x$ has been matched so far.)
%% 	\item For $i=1$ to $mx * k_1$ do:   \# for $mx * k_1$ we can use \algproblemrone{} algorithm %for at least one k times
%% \item	Divide $X$  into sets, $A_1,A_2, \ldots, A_m$  according to the value of $e_x-r_x$, such that $A_1$ is the set with minimum value and $A_m$ is the set with maximum value. (it is possible to union all sets with $e_{x_i }-r_{x_i} \geq 0$).
%% \item	Find a maximum matching $M_1$ with only the agents in $A_1$. Find another maximum matching, $M_2$ in $(A_1 \cup A_2,Y,E_2)$ ; start with $M_1$ and extend it by finding augmenting paths 
%% (as in Hopcroft-Karp algorithm \cite{Hopcroft-Karp-1973}).
%% 	Continue in that manner until  $M_m$ has been constructed.
%% \item	For each $(x,y)$ in $M_m$,
%% 	  $e_x=e_x+1$ 
%% 	(If we want exactly $\rho_x$ matchings for each agent $x$, remove all agents with enough matchings, it saves time)
%% \item	If $\forall x$,$e_x-\rho_x \geq 0$, return $i$
%% \item	Return $mx * k_1$
%% 	\end{enumerate}
%% \caption{Steps of our heuristic for \problemprb{}}
%% \label{fig:heu_gen_prob}
%% \rule{\columnwidth}{0.01in}
%% \end{figure}
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Idea:}~ We will formulate the ILP for \problem{} so that the subgraph (of the compatibility graph)
resulting from the solution is \emph{not} a matching but one
in which the degree of agent node $x_i$ is at least $\rho_i$.
We will add constraints to ensure that in each round, each agent
is matched to at most one resource.
We will also ensure through appropriate constraints that 
in each round, each resource is assigned to at most one agent.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
%These constraints will ensure that we can easily decide in which rounds 
%a given agent will be matched; further, given an agent and a round,
%we can also determine the resource to which
%the agent will be matched in that round.

%\medskip

%\noindent
%\textbf{ILP Formulation:}~ 

%medskip

\subsection{\problemprb{}: A variant of  \problem}
\label{sse:def_each_round_budget}

We also consider a variant of \problem, 
denoted by \problemprb{}, where the budget $\beta_i$
specified for each agent $x_i$ is for \emph{each round}
of matching.
Thus, the difference between \problemprb{} and \problem{} 
is that in the latter, the budget is the upper bound on
the cost incurred by an agent \emph{over all the rounds}.
Except for this, the specifications of the decision and
minimization versions of \problem{} and \problemprb{}
are identical.

Because of the difference in the way the budget 
is interpreted in \problem{} and \problemprb{},
it easier to construct the compatibility graph for the  \problemprb. To see why,
notice that for \problem{},  the edges in the compatibility graph can be constructed only after the labels removed
by all the agents are known.
For \problemprb, an agent $x_i$ can consider each incident
edge in the restrictions graph and add it 
to the compatibility graph if the cost of
removing the labels on that edge is at most the budget.
This is possible because each such edge meets the
budget constraint and an agent uses
at most one edge in each round (matching).
Therefore, when considering \problemprb{}, we may
assume that the input is the compatibility graph
(instead of the restrictions graph).


%% We first describe the datasets used and the
%% experiments framework. For the ILP implementation, we used \cite{coinor}.
%% For evaluation we considered the minimization versions, the minimum number
%% of matchings~$k$ required and the computation time.

%% \subsection{Summary of results}
%% \label{sse:summary_res}

In this work, we establish complexity results and develop several
algorithms for the \problem{} and \problemprb{} problems. We experiment
with novel real-world datasets and synthetic data to study the performance
and utility of the algorithms. A summary of our contributions is as follows.

%% 
%%      
%% 
%% \medskip
%% 
%% \noindent
%% \textcolor{red}{(Need to use or remove the following
%% bullet points.)}
%% 
%% \begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
%%     \item Resource allocation problems have been studied
%%      by many AI researchers in the context of multi-agent systems.
%%      
%%      \item There may be no resource that is compatible with the capabilities desired by an agent; so, an agent needs to relax its requirements before it can be matched to a resource. However, such a relaxation incurs a cost for the agent (due to regret) and each agent has a budget on the cost.
%%      The focus of the paper is on generating advice regarding such relaxations to agents.
%%     
%%     \item Since number of resources is usually (much) less than the
%%     number of agents, in general, several rounds of matching are needed for all agents to be matched.
%%     \item We formulate several optimization problems that arise in the context of relaxing agents' requirements with budget constraints so that all agents can be matched within a few rounds.
%%     \item Our results establish the complexity of the general problem. We also present efficient algorithms for a restricted version, an ILP formulation and an efficient heuristic for the general version.
%%     \item We demonstrate the usefulness of our approach using two real data sets, namely matching instructors to classrooms and matching children to
%%     recreational activities.
%% \end{itemize}

%% An agent may be reluctant to relax too many preferences. Therefore, we
%% assume that there is a cost for each relaxation and that each agent has a
%% budget on the total relaxation cost.
%% Many applications require agents to be matched to resources whose
%% specifications are compatible with agent preferences. In such a case, the
%% system or a \prin{} must generate suitable advice for the unmatched agents
%% so that agents who heed the advice can be matched to resources. The advice
%% provided by the \prin{} consists of relaxations of the agent's preferences.
%% An agent may be reluctant to relax too many preferences. Therefore, we
%% assume that there is a cost for each relaxation and that each agent has a
%% budget on the total relaxation cost.  After appropriate relaxations
%% satisfying the budget of each agent are identified, the compatibility
%% relationship between agents and resources can be represented by a bipartite
%% graph $G(X, Y, E)$, where node sets $X$ and $Y$ represent the agents and
%% resources respectively and each edge $\{x, y\}$ indicates that agent $x$ is
%% compatible with resource $y$.  Each matching of $G$ represents an
%% assignment of resources to agents.  Since the number of available resources
%% is generally much smaller than the number of agents, several rounds of
%% matching may be necessary to assign a compatible resource to each agent.
%% We study some optimization problems that arise in this context.  One
%% problem involves finding the minimum number of rounds of matching so that
%% each agent can be matched to a resource at least once and the cost of the
%% required relaxation for each agent is at most the agent's budget.  We show
%% that this problem can be solved efficiently.  A more general version is to
%% find the minimum number of rounds of matching so that each agent is matched
%% a specified number of times while satisfying the budget constraint.  We
%% show that this problem is NP-hard and present several practical approaches
%% (e.g., an integer linear programming formulation, a heuristic using
%% simulated annealing) to cope with its computational intractability.  We
%% experimentally evaluate our methods on synthetic networks and apply them to
%% two real-world situations: matching courses to classrooms and children to
%% activities.
\begin{itemize}
    \item Only a placeholder. Hopefully will have something by the end of our holiday.
\end{itemize}
\label{local_search}
\end{figure}
\begin{figure}
\includegraphics[scale=0.5]{figures/local_search.png}
\caption{\aacomment{is this required?} General budget; looking for optimal relaxation, changing agents that needs more than 2 matching; in this case 10. for different budgets.}
\label{local_search}
\end{figure}

\begin{figure}
%%% Temporarily commented out by Ravi (so that latex can
%%% produce an output pdf.
%\includegraphics[scale=0.5]{figures/does not exist}
\caption{General budget; looking for optimal relaxation, changing agents that needs more than 2 matching; in this case 10. budget =2, compare local search and ILP}
\paragraph{ILP vs Heuristic}

Running the heuristic may take few minutes , ilp may even few days.

The quality ?
%\begin{itemize}
 %     \item x axis is the agents with demand in {5,10,15,20} rest are with demand of 2 matchings.
  %  \item different values of k for ilp and greed heuristics.
   % \item 10 datapoints for different percents.
    %\item high requirement agents are chosen randomly 100 times and average is calculated.
    %\item graph is after relaxation with budget of 2.
    
%\end{itemize}



\paragraph{Budget sufficient for each matching separately}
In Figure~\ref{school_k} and figure~\ref{class_k} we compared between the ILP and the heuristic for finding how many matchings are need to satisfy the agents' requests where the budget should be sufficient for each matching separately. In \ref{school_k} we study the children Summer Vacation
Activities and in Figure~\ref{class_k} we refer to the class room data set. That is the agents refer to children and courses  respectively and resources refer to activities and classes, respectively. 
In Figure~ \ref{school_times} and \ref{class_times} we report the time needed for these settings for the children activity and the courses datesets respectively.

\begin{figure}
\includegraphics[scale=0.5]{figures/school_times.png}
\caption{Budget for each matching, school time}
\label{school_times}
\end{figure}
In Figure~ \ref{school_times} we ran:
\begin{itemize}
    \item run time for greedy and ilp
    \item using cbc solver. tried also gurobi which considered as state of the art.
    
\end{itemize}
\begin{figure}
\includegraphics[scale=0.5]{figures/class_k.png}
\caption{Budget for each matching, courses, k}
\label{class_k}
\end{figure}
In Figure~ \ref{class_k}:
\begin{itemize}
    \item Same definitions but for courses and classes
\end{itemize}

\begin{figure}
\includegraphics[scale=0.5]{figures/class_times.png}
\caption{Budget for each matching, courses,time }
\label{class_times}
\end{figure}
In Figure~ \ref{class_times}:
\begin{itemize}
    \item Same definitions but for courses and classes
\end{itemize}
\begin{figure}
\caption{General budget, random graph; different probability.at least 1, k as a function of m }
\label{random_k}
\end{figure}
In Figure~\ref{random_k}

\begin{itemize}
    \item Relaxing 0.0,0.2,0.4,0.6,0.8 or 1.0 of the constraints for each relevant attribute.
    \item Remove agents with no edges in the beginning.
    \item save runtimes as well
    \item choose k by using algorithm of at least one.
\end{itemize}
\begin{figure}
\includegraphics[width=\columnwidth]{figures/relax_course_class.pdf}
\caption{General Budget, courses increasing budget and its effect on different attributes, at least one}
\label{relax_course_k_1}
\end{figure}
\begin{itemize}
    \item Random graphs. agents are chosen among large initial set  such that they will have at least 1 edge.
    \item No requirement from the resources.
    \item 4 data points, 100,0.75,0.5,0.25
    \item run massively in parallel, 1000 times per option.
    
\end{itemize}
%% We study how the the budget and $\tau$ influence $k$ and the time and we
%% also considered the problem where each agent needs to participate in at
%% least one matching.
%% We considered two real-world detests and  random graphs.
The first
set of experiment results corresponds to \problemrone, followed by results
for \problemprb{} where we compare
\ilpproblemprb{} with \greedyproblemprb. The third set 
corresponds to the general \problem{} where we compare \ilpproblem{} with
\greedyproblem. 

\medskip

\noindent
\textbf{Problem Statement:} (Decision Version)

\noindent
\underline{\textsf{Given:}}~ A restriction graph $G_R(\agset, \rset, E_R)$; 
for each agent $x_i$, 
two positive integers $\beta_i$ (budget on the total cost of removing labels) and
$\rho_i$ (the minimum
number of times $x_i$ should be matched), $1 \leq i \leq n$;
for each edge $e = \{x_i, y_j\} \in E_R$, a subset $\Gamma_e \subseteq \calc_i$
of labels;
for each label $c_{i,t}$, a cost $\psi_{i,t}$ of removing
that label, $1 \leq t \leq \ell_i$ and
$1 \leq i \leq n$;
a positive integer $k$ (the upper bound on the number of rounds
of matching).

\smallskip

\noindent
\underline{\textsf{Requirement:}}~ For each agent $x_i$, is there a 
subset $\calc'_i \subseteq \calc_i$ such that the following
conditions hold?
\begin{description}
\item{(i)} The cost of removing all the labels in $\calc'_i$ for agent $x_i$
is at most $\beta_i$, $1 \leq i \leq n$, and 
\item{(ii)} the compatibility graph \compgr{} resulting 
from the removals of labels has a collection of at most $k$ matchings
$M_1$, $M_2$, $\ldots$, $M_k$, with agent $x_i$ appearing in at least
$\rho_i$ of these matchings.
\end{description}
%(We need \emph{not} produce a maximum matching in each round.)




the general version of the problem for minimizing the number of rounds
when some agents need to be matched two or more times.
Further, for each agent, the total cost of relaxation 
over all the rounds must be within the agent's budget.



We will consider scenarios where~$\rho(\cdot)$ is a constant function. In
such cases, we will use the notation~$r$ to refer to this constant and
denote this special case as~\problem$(G_R,\cost,b,k,r)$.
Given a restrictions graph~$G_R(\agset\cup\rset,E_R)$ coresponding
to~$n_{\agset}$ agents~$\agset$ and~$n_\rset$ resources~$\rset$ with
agent-specific restrictions defined by~$E_R$, a
function~$\cost(\cdot)$ that defines the cost incurred in removing a subset
of agent-specific restrictions, budget~$b:\agset\rightarrow\integers$,
number of rounds~$k$ and minimum number of matchings
$\rho:\agset\rightarrow\integers$.
\smallskip

\noindent
\textbf{Problem.} For each agent~$x$, find a set of
restrictions~$C\subseteq C_x$ to remove such that~$\cost(C_x)\le b(x)$ and
the resulting compatibility graph~$G_C$ has~$k$ matchings where each
agent~$x$ is matched at least~$\rho(x)$ times. 

:~\tikz[baseline=-.5ex]{\node
(x) {$x_i$}; \node at (1,0) (y) {$y_j$}; \draw (x) --
node[label=above:{\scriptsize $C$},shift={(0,-.15)}]{} (y)}



se have formulate the problem of multi-round matching
generating advice (i.e., suggesting relaxations of agents' requirements) so
that all agents can be matched to resources using a minimum number of
rounds. (Each round allows a subset of agents to access resources.)
\noindent
\textbf{Multi-round matching with advise.} We describe a multi-round
resource allocation problem called~\problem{} where
a set of agents are matched to resources given agent restrictions and
resource specifications in a specified number of rounds. Relaxation of each
restriction incurs a cost. The objective is
to advise agents to relax certain restrictions in order to match resources

Let~$\setc'\subseteq\setc$ be a solution to the set cover instance. This
means that there exist~$\alpha$ subsets that cover~$U$. We will remove the
corresponding labels in~$G_R$. Since~$\setc'$ covers all elements in~$z_j
\in U$,~$\exists A_h\in \setc'$ that contains it. This implies that there
is no label on the edge~$y^j_h$. The special agent~$x^*$ can be matched to
one such~$y^j_h$ in each matching.  For any~$z_j\in U$, since there are
only~$k\cdot\deg(z_j)-1$ agents in~$\agset^j$ all of which are adjacent
to the same set of~$\deg(z_j)$ resources, there are enough resources to match
each~$x\in\agset^j$ in some matching.


For each agent~$x$, there is a cost
associated with removing restrictions. Let~$\cost: 2^{C_x}\rightarrow \reals$
be a mapping of each subset of agent~$x$'s constraints to a real number.


Each resource in \rset{} is
associated with a collection of \emph{attributes}, and
each attribute takes on values from a finite domain. 
Every agent would like to be matched to a resource. 
However, agents may have
\emph{preferences} that prevent them from being matched to certain
resources. Such agent-resource pairs are said to be \emph{incompatible}. The problem of assigning
resources to agents can be seen
as a \emph{maximum matching problem} \cite{CLRS-2009} on a \emph{bipartite graph}
$G(\agvset, \rvset, E)$, where the node sets \agvset{} and \rvset{}
correspond to agents and resources respectively and each
edge $\{u,v\} \in E$, with $u \in \agvset$ and $v \in \rvset$,
indicates that the agent represented by $u$ is compatible
with the resource represented by $v$.
We refer to $G$ as the \textbf{compatibility graph}.
%with one part comprising of nodes representing agents and the other part
%representing resources. There is an edge between an agent and a resource if
%and only if they are compatible.
\emph{While the matching problem on $G$ plays a role in our work, 
our focus is not on that problem.}

We will use the following running example of matching courses  to
classrooms.  Each classroom is a resource and each course (or its
instructor) is an agent. Classrooms have three attributes: capacity, region
(building or division) and accessibility (i.e., whether it can accommodate
students with disabilities).  For each classroom, the values of these
attributes represent the constraints associated with that classroom.  Each course has preferences such as the required minimum and maximum capacity
values, preferred regions, and whether it requires an accessible classroom.

Formally, let~$\agset =\{x_1,x_2,\ldots, x_n\}$ be a set of~$n$ agents
and~$\rset =\{y_1,y_2,\ldots, y_m\}$ be a set of~$m$ resources. 

Each resource is characterized by a finite set of~$\alpha$ attributes. It is
assumed that each attribute can take on a finite set of values and that these values can be either symbolic or discrete. The values of $y_j$'s attribute, $a$, are denoted as $y^a_{j}$. The vector of attribute values for a resource $y_j$ is denoted as $b_j$.

Each agent~$x_i$ expresses its preferences as personal ordering, capacity with lower and upper bounds and binary decision.
The personal ordering threshold is modeled as the threshold function- $t(f_i(y^a_{j}),0)=f_i(y^a_{j})>0$. For this function, the attribute values are symbolic. The symbolic values are converted to real values according to the personal preferences of agent~$x_i$ and the maximum among them is chosen using $f_i$.

Regarding the binary decision, the possible attribute values are $\{-1,1\}$ and the threshold function is one of $t(f_i(y^a_{j}),0)$ and $t(f_i(-y^a_{j}),0)$ where $f_i$ is choosing the maximum value among the values of $y^a_{j}$.
Capacity is modeled as a couple of threshold functions; A set of two thresholds, $5<=x^a_{i}<=10$, is written as $t(f_i(y^a_{j}),5)$ and $t(f_i(-y^a_{j}),-10)$ where like before, $f_i$ is choosing the maximum among values of $y^a_{j}$.
The whole preference set of an agent, including the $f_i$ function for converting symbols to real numbers is defined as a conjunction of threshold functions denoted as $\kappa_i = \{R|S\}^\alpha \longrightarrow \{0,1\}$. In case when all clauses of the conjunction function belong to the binary decision class, the conjunction of threshold functions could be modeled as a simple conjunction of Boolean variables.
\\

\noindent
\textbf{Example 1:}~
We now illustrate the above definitions using the course-classroom example. Suppose each classroom has a
capacity between~$10$ and~$50$ in steps of 10, and there are four regions numbered~1 through 4.
Here, we have two attributes ($\alpha=2$).  
Let~$y_1$ be a
classroom in region~$'3'$ with capacity~$30$ and~$y_2$ be a classroom
in region~4 that can accommodate courses of size ~$50$. 
Suppose the instructor
for the course~$x_1$ has the following preference over the regions- $(4,2,3,1)$ and requires that the selected region will be $>=3$. Suppose also that the instructor requires that the capacity will be in the range ~$20$ and~$30$.
The corresponding
compatibility function is 
$\kappa_1=(20 \leq c \leq 30) \And (~3\leq f_i(r))$ for $c=30$ and $r='3', f_i('3')=3$ and in more formal way,$\kappa_1(b_1) =1$ for $b_1=(30, '3')$.

Note that~$x_1$ is compatible with $y_1$; 
in fact, $x_1$'s preferences satisfy both the capacity and region
constraints of $y_1$.
However, $x_1$ is not compatible with ~$y_2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{The advice framework.}
The following are the steps in the maximum matching advice framework.
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item Every agent $x_i$ in~$\agset$ sets its preferences by specifying the thresholds and the $f_i$ function in $\kappa_i$.

\item For each agent-resource pair $(x_i,y_j)$,
if~$\kappa_i(b_j))=1$, we add the edge $\{x_i,y_j\}$ to the
compatibility graph $G$.
\item The nodes are ordered deterministically and the \hk{} algorithm is applied.
\item Few unmatched agents approach the \prin{} with the query as to why they were not matched.
\item For each unmatched agent, $x_i$, the \prin{} adds to the compatibility graph, $G$, all edges that fulfil a budget constraint specified by agent $x_i$.
\item Then, the principal is running again the \hk{} algorithm:
\begin{itemize}
        \item With only the unmatched agents and resources.
        \item With all agents and resources
        \item with all agents and resourses, starting with matching only previously matched agents and then augmenting that matching.
        According to the proof of $\hk{}$, it is guaranteed that the resulting matching will be a maximum matching that contains all previously matched agents.
\end{itemize}
\item Finally, for each matched agent among the approaching agents, the \prin{} suggests to relax the relevant constraint as a \problem{}.
\end{enumerate}

%%
We now introduce certain concepts related to the last few steps above
and formulate the \problem{} problem.
%%
\paragraph{The advice framework alternative.}
The following are the steps in the maximum matching advice framework.
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item Every agent $x_i$ in~$\agset$ sets its preferences by specifying the thresholds and the $f_i$ function in $\kappa_i$.

\item For each agent-resource pair $(x_i,y_j)$,
if~$\kappa_i(b_j))=1$, we add the edge $\{x_i,y_j\}$ to the
compatibility graph $G$.
\item The nodes are shuffled and the \hk{} algorithm is applied.
\item Few unmatched agents approach the \prin{} with the query as to why they were not matched.
\item The \prin{} creates a new empty compatibility graph $G\prime$ with the unmatched nodes and the unmatched resources as nodes. 
\item Then, for each matched agent among the approaching agents, the \prin{} suggests to relax some constraints as a \problem{}.
\item According to the decision of the remaining agents, the \prin{} adds to the new compatibility graph, $G'$, all new compatible edges.
\end{enumerate}

%%
We now introduce certain concepts related to the last few steps above
and formulate the \problem{} problem.
%%

\paragraph{Suggesting changes to~$\kappa_i$ through extensions.} The
objective is to suggest modifications to the compatibility function in such
a way that any resource that is already compatible (but unmatched)
continues to be compatible with the agent, and additional resources become
compatible as a result of the modifications.
Such modifications increase the chances
of the agent being matched. Therefore, we will consider only modifications that
satisfy the following property: $\kappa'_i$ is an \textbf{extension}
of~$\kappa_i$; i.e., for any input~$b_j$,~$\kappa_i(b_j)=1$ implies that~$\kappa'_i(b_j)=1$.

Continuing with our course-classroom example, there are two ways to obtain
an extension of~$\kappa_1$: we can either increase threshold bound or remove it totally. For instance, 
$\kappa'_1= (20 \leq c \leq 60 )$ 
is an extension of~$\kappa_1$ considered in Example~1.
It was obtained by replacing the current threshold of $30$ with the new threshold- $60$ and removing the region preferences threshold. 
Now,~$x_1$ is compatible with~$y_2$ also.

\paragraph{Cost and benefit of extending~$\kappa_i$.} For each attribute~$a\in
\attribs$, we will assign a cost~$\chi(a)$ for changing its value in one step. If~$a$ is untouched, then, no cost is incurred. 

The benefit of extending~$\kappa_i$ to~$\kappa'_i$ is  having ~$x_i$ matched in some cases.

We are now ready to define formally the advice framework. Given a set of
agents~$\agset$, resources~$\rset$, attributes ~$\attribs$ and
the compatibility graph~$G(V_\agset,V_\rset,E)$, the advice framework
for agents~$x_i...x_j$ is denoted
by~$\framework(\attvec_i,\kappa_i,\chi)$,
where~$\attvec_i{(\cdot)}$ is
the attribute function,~$\kappa_i$ is the
current compatibility function of~$x_i$ and~$\chi(\cdot)$ is the cost
function. Now we define the \problem{} problem.

\begin{definition}[Problem {\normalfont \problem}]
For a set of customers~$\{x_i...x_j\}\in X$ with advice
frameworks ~$\framework(\attvec_i,
\kappa_i,\chi)$ and
budgets~$\beta_i$, find~$\kappa^*_i$ that maximizes benefit with costs $\leq$ $\beta_i$;.
\end{definition}
Suppose there are two
sets of restrictions~$C$ and~$C'$ such that if either one of them is
removed,~$x$ becomes compatible with~$y$, then, we draw two separate edges
between them with one lableled~$C$ and the other~$C'$. 

Numbers:
AND: Average(maximum(0,Exhaustive probability - Greedy))=0.016, stdev= 0.06837. min(pi +)  for the greedy and exhustive algorithm were 0, 0  and max values were 1 and 1.
OR: Average(maximum(0, Exhaustive probability - Greedy))=0.0085, stdev= 0.01256. min(pi +) for the greedy and exhustive algorithm were 0.502 and 0.485 and max values were 1 and 1.
The parameters with greatest covariance were B (0.02 in AND and 0.0007 in OR) and resources_amount( -0.03 and 0.0036) .
For the AND case I run ~300 experiments when setting the other parameters to some constant value. I found that when the world (B) is greater, the error is also greater. I couldn't have the same findings on the OR case since the greedy and the exhaustive gave very similar probabilities.
A graph for the AND case with |B| as the X axis, is available on the sup_figures folder(with some more heatmaps and the graph with the distinct number of resources per 100 when having different amounts of attributes and values).

Parameters that were used for the AND case for verifying the effect of B were:  R=1, Gamma=3, #of resources=40.
and (ii)~evaluation of the algorithms developed for the \problem{} under
different explanation frameworks.

\begin{figure}[t]
\centering
\begin{tabular}{cc}  
\includegraphics[height=2.5cm,width=0.5\linewidth]{figures/theta1_change_2.png}&
\includegraphics[height=2.5cm,width=0.5\linewidth]{figures/theta2_change_2.png}\\
\multicolumn{2}{c}{\includegraphics[height=2.5cm,width=0.5\linewidth]{figures/p_change_2.png}}
\end{tabular}
\caption{Uno vs Hopkroft} 
\label{fig:exp_utility_cmp}
\end{figure}

\begin{itemize}
\item We run each experiment 1000 times
\item Results for 10*10 random graphs were considered. We tried also {5-15}*10 graphs with no important conclusions.
\item For each graph class the parameters for $\theta_hk$ were different.
\item For measuring our results on larger graphs we run the hk-uno algorithm with different parameters on the real dataset and on larger random graphs(e.g., $40*40$ and $80*40$. Here we couldn't calculate the true probabilities because it can take forever. We therefore assumed that lower variance may predict on better parameter set. We found that increasing the number of uno iterations is not improving the variance while the number of hk improves it linearly. That was the reason for using only Hopkroft iterations in the relaxation problem.
\item Runtime of Hopkroft was significantly longer than of a single Uno iteration. HK as a preference because it can run in parallel.
\end{itemize}


\paragraph{Datasets.}
\subsubsection{Children School Vacation.}
A real dataset ~\cite{varone2019dataset}, based on online registration during the summer of 2017 for assigning holiday activities to children.
Each activity has a relevant age range. In addition, dataset contains some children preferences. Some of the activities were very expensive and therefore a child was permitted to participate in them only once in her life. There were three holiday periods in the dataset. Authors suggested a linear program for solving the relevant optimization problem in the case when assigning at most one activity per child is permitted.
\begin{itemize}
\item 634 children participated.
\item there were three vacation period. I picked the one that started at 09/10/2017 0:00 and ended at 15/10/2017 0:00.
\item there were 249 relevant activities in the relevant period (out of 496 in total).
\item Attribute Preferences has the values: 1,2,3,4,5. 1-4 are explicit ratings that provide partial order.
and 5 is when there is no such rating. I assumed that 5 is worse than the other 4 for having a complete order.
\item Attribute min age with values 6-15
\item Attribute max age with values 7-16
\item I did not use the lifetime attribute in the school children case because it was very rare and with no important meaning.
\item There were 3 distict vacation periods in the graph, I picked one of them.
\item I added all children to the matching.
\item The most relaxed parameter was the preference. In many cases it was relaxed to 5. It means that they need to find a way to increase number of ratings for having better idea about the preferred activities. 
\end{itemize}
\subsubsection{Courses and classrooms graphs}
Although the problem of assigning classrooms to courses is quite common ( e.g., ~\cite{phillips2015integer} ) we couldn't find a dataset that is good for our needs. We collected a new classroom assignment dataset from
a university on 2018-2019 \footnote{Additional information about
the data set will be provided in the final version of the paper}. For each of the 144 classrooms, a region in the university and total student capacity is given. In addition, each classroom has details about its available disability accessories. For many of the courses there were specific region preferences. Since we couldn't find real details about people with disability, we generated the relevant data randomly, giving a course 10 percents for needing one of the accessories and 1 percent for needing both.

\begin{itemize}
\item We have the Capacity attribute with values from 16 to 270
\item there are also the region attributes with values {1100,900,200,400,500,300,100,1000 }
\item As discussed, their order was determined randomly.
 
\the hearing and accessible attributes were generated randomly as before.

\item 144 rooms
\item I picked all courses that used at least part of the window of Tuesday, 14:00 pm- 16:00 pm.
\item I filtered out randomly about 40 percents of the rooms for having lower matching probabilities.
\item The administrator said that they have to keep 20 percents of the rooms empty for some events.
\item The initial number of courses in the time-range is 154.

\end{itemize}

\subsection{Evaluating \hkuno{} algorithm.}

The main objective was to assess the quality of the algorithm.
For the \rhk{} algorithm, we used the implementation of the python networkx package~(\citeyear{SciPyProceedings_11}). For the Uno~(\citeyear{uno1997algorithms}) iterations, we used a github implementation. \footnote{https://github.com/Xunius/bipartite\textunderscore matching} as a basis. For making the implementation simple we did not implement the suggested speed up improvements.
For measuring the quality of the \rhk{} algorithm and determining its parameters we generated a large set of random graphs. Graphs differ in their $P$ values, which is the probability of an edge to exist. They also differ in the number of the nodes in each of their parts. For each graph and for each of its nodes, the ~$\empprob$ was calculated by using \rhk{} with different parameters. The results were averaged over multiple nodes and multiple graphs and compared to the ~$\trueprob$ by using the Uno~(\citeyear{uno1997algorithms}) algorithm. 
\begin{figure}
\includegraphics[height=6cm,width=9cm]{figures/0.35_10_10_1000.png}
\caption{An example heatmap that shows the Average MSE in a set of $1000$ random graphs with $P=0.35$, $n=10$ and $m=10$. The y axis represents $\nhk$ and the x axis represents $\nuno$. The brighter squares indicate greater mistakes. }
\end{figure}

\subsection{Performance of the algorithms for calculating ~$\frameworkand$\label{alg:and_greedy} and ~$\frameworkand$\label{alg:or_greedy} on synthetic graphs.}
\begin{itemize}
\item For both the AND and OR cases, I used the parameters: R= values per Attribute,{1..5}
                       B= world size, {2,4,6,8,10,12}
                       Gamma= preferences size, { 1..5 }
                       Resources amount, {20,40}
                       Budget { 1...5 }
                       
\item for the AND case, the average difference between the greedy heuristic and the exhustive search was 0.02 for all 6921 experiments. 
\item In my implementation, I called the oracle for each set of relaxed resources (1 or more) without checking if it increased the matching size.
\item In the OR case there was no significant difference. Actually the greedy was better in 0.001 percents (negligible because of the error).
\Item I found that as the world (B) is greater, the error is also greater.

\end{itemize}                       

\subsection{Performance of the algorithm for calculating ~$\frameworkth$\label{alg:thresh} on the real datasets.}
>>>>>>> 9b9805c8d9813b8318c8eabf60ef4957b5e7121e

\begin{itemize}
\item I picked all courses that used at least part of the window of Tuesday, 14:00 pm- 16:00 pm.
\item I filtered out randomly about 40 percents of the rooms for having lower matching probabilities.
\item The administrator said that they have to keep 20percents of the rooms empty for some events.
\item The initial number of courses in the time-range is 154.

\end{itemize}
%% Some of the activities were very expensive and therefore a
%% child was permitted to participate in them only once in her life. There
%% were three holiday periods in the dataset. Authors suggested a linear
%% program for solving the relevant optimization problem in the case when
%% assigning at most one activity per child is permitted.
%% \begin{itemize}
%% \item Attribute Preferences has the values: 1,2,3,4,5. 1-4 are explicit ratings that provide partial order.
%% and 5 is when there is no such rating. I assumed that 5 is worse than the other 4 for having a complete order.
%% \item Attribute min{\_}age with values 6-15
%% \item Attribute max{\_}age with values 7-16
%% \item I did not use the lifetime attribute in the school children case because it was very rare and with no important meaning.
%% \item There were 3 distict vacation periods in the graph, I picked one of them.
%% \item I added all children to the matching.
%% \end{itemize}

\begin{itemize}
\item We run each experiment 1000 times
\item Results for 10*10 random graphs were considered. We tried also {5-15}*10 graphs with no important conclusions.
\item For each graph class the parameters for $\theta_hk$ were different.
\item For measuring our results on larger graphs we run the hk-uno algorithm with different parameters on the real dataset and on larger random graphs(e.g., $40*40$ and $80*40$. Here we couldn't calculate the true probabilities because it can take forever. We therefore assumed that lower variance may predict on better parameter set. We found that increasing the number of uno iterations is not improving the variance while the number of hk improves it linearly. That was the reason for using only Hopkroft iterations in the relaxation problem.
\item Runtime of Hopkroft was significantly longer than of a single Uno iteration. HK as a preference because it can run in parallel.
\end{itemize}


The main objective was to assess the quality of the algorithm.  For the
\rhk{} algorithm, we used the implementation of the python networkx
package~(\citeyear{SciPyProceedings_11}) and for the ``Uno'' component of
the algorithm we used a github
implementation\footnote{https://github.com/Xunius/bipartite\textunderscore
matching} as a basis. For making the implementation simple we did not
implement the suggested speed up improvements.  For measuring the quality
of the \rhk{} algorithm and determining its parameters we generated a large
set of random
graphs. Graphs differ in their $P$ values, which is the probability of an
edge to exist. They also differ in the number of the nodes in each of their
parts. For each graph and for each of its nodes, the ~$\empprob$ was
calculated by using \rhk{} with different parameters. The results were
averaged over multiple nodes and multiple graphs and compared to the
~$\trueprob$ by using the Uno~(\citeyear{uno1997algorithms}) algorithm.

Parameter sets for both AND and OR cases:
R= values per Attribute,{1..5}
B= world size, {2,4,6,8,10,12}
Gamma= preferences size, { 1..5 }
Resources amount, {20,40}
Agents amount, {40 for 20 resources and 80 for 40 resources}
Budget { 1...5 }


==> yohai_rawlsian.tex <==
%%%%%%%%%%%%%%%. This is Yohai's version. %%%%%%%%%%%%
\subsection{Maximize Minimum allocation}

\begin{enumerate}[leftmargin=*]
	
\item $Q=\{k_1/k_2 ~|~,k_1\in[0..k],k_2\in[1..k],k_1\leq k_2\}$
\item $Q = unique(reverse(sorted(Q)))$
\item $ord: Q -> N$ is a function that returns for each item in $Q$ its position in $Q$.
\item $\xi: Q\rightarrow N$, $\xi(j)=(k\cdot n)^{ord(j)}$
\item $\xi_{max}=max_{q\in Q}(\xi(q))$
\item $\xi^*:Q\rightarrow [0,1],\forall{q\in Q}, \xi^*(q)=\xi(q)/\xi_{max}$.
\item $\mu_i: [1,2,..\rho_i]\rightarrow R$, $\mu_i(l)=\sum_{o=0}^{l-1}\xi^*(o/rho_i)$ if $l>0$ else $0$
\end{enumerate}

\begin{lemma}
$\forall{i}, \mu_i(\cdot)$ satisfies diminishing returns property
\end{lemma}

\begin{proof}
We show that $\mu_i(h)-\mu_i(h-1) \leq \mu_i(h-1)-\mu_i(h-2)$.\\
\\
\noindent
\textbf{Case 1}: $h\geq3$:\\
Following definition:
$\mu_i(h)=\sum_{l=1}^{h-1}\xi^*(l/\rho_i)$,
$\mu_i(h-1)=\sum_{l=1}^{h-2}\xi^*(l/\rho_i)$,
$\mu_i(h-2)=\sum_{l=1}^{h-3}\xi^*(l/\rho_i)$.\\
Therefore, $\mu_i(h)-\mu_i(h-1)=\xi^*({h-1}/\rho_i)$ and similarly $\mu_i(h-1)-\mu_i(h-2)=\xi^*({h-2}/\rho_i)$.
Since $(h-2)/\rho_i<(h-1)/\rho_i$, $ord(h-2/\rho_i)>ord(h-1/\rho_i)$
and also $\xi(h-2/\rho_i)=((k)\cdot n)^{ord(h-2/\rho_i)} >\xi(h-1/\rho_i)=((k)\cdot n)^{ord(h-1/\rho_i)}$. Finally, $\xi(h-2/\rho_i)>\xi(h-1/\rho_i) \rightarrow \xi^*((h-2)/\rho_i)>\xi^*(h-1/\rho_i)$ and we are done.\\
\\

\noindent
\textbf{Case 2}: $h=2$:\\
Following definition:
$\mu_i(h)=\sum_{l=1}^{h-1}\xi^*(l/\rho_i)$,
$\mu_i(h-1)=\sum_{l=1}^{h-2}\xi^*(l/\rho_i)$,
$\mu_i(h-2)=((k)\cdot n)^{k^2}$\\
Therefore, $\mu_i(h)-\mu_i(h-1)=\xi^*({1}/\rho_i)$.
Regarding the right side, $\mu_i(h-1)-\mu_i(h-2)= \mu_i(1)-\mu_i(0) = \xi^*({0}/\rho_i)$.
And we continue similar to case 1.
\end{proof}

\begin{lemma}
$\forall{i},\forall{ h\in[1..k]},  0 \leq \mu_i(h)-\mu_i(h-1) \leq 1$ 
\end{lemma}
\begin{proof}
Follows directly from the normalization in line 4
\end{proof}

\begin{theorem}
(weak version)
Given a multi-round solution~$\mbsoln$ that maximizes $\totreward(\mbsoln)=\sum_{i=1}^n\reward_i(\ell_i)$, $\mbsoln$ also maximizes 
$min_{x_i, 1\leq i \leq n}\ell_i/\rho_i$.
\end{theorem}

Proof:
Let $x_o=min_{x_i, 1\leq i \leq n}\ell_i/\rho_i$.
For each agent $x_i, 1\leq i \leq n$, ${{\ell_o}_i}=\min \{\ell_i,\min \{j~|~ j/\rho_i> \ell_o/\rho_o\}$.
Let $C_1=\sum_{i=1}^n\reward_i({\ell_o}_i)$ and let $C_2=\sum_{i=1}^n\reward_i(\ell_i)-\reward_i({\ell_o}_i)$. We note that $C_1+C_2 =\sum_{i=1}^n\reward_i({\ell_o}_i) + \sum_{i=1}^n\reward_i(\ell_i)-\reward_i({\ell_o}_i)= \sum_{i=1}^n\reward_i(\ell_i)=\totreward(\mbsoln)$.
Assume by negation that $\mbsoln$ maximizes $\sum_{i=1}^n\reward_i(\ell_i)$ but not $min_{x_i, 1\leq i \leq n}\ell_i/\rho_i$. 
Let $\mbsoln'$ be a multi-round solution that maximizes $min_{x_i, 1\leq i \leq n}\ell'_i/\rho_i$ where for each agent $x_i, 1\leq i \leq n$, $l'_i$ is the number of rounds assigned to $x_i$ in $\mbsoln'$.
We first define $C_1',C_2'$ as they were defined for $\mbsoln$.
We show that $\totreward(\mbsoln')>\totreward(\mbsoln)$, contradicting the assumption that $\mbsoln$ maximizes $\totreward(\cdot)$.

First, $\delta_o(\ell_o+1)=\xi^*(\ell_o/\rho_o)$ (by definition).
In addition, $C_2=\sum_{i=1}^n\reward_i(\ell_i)-\reward_i({\ell_o}_i)=\sum_{i=1}^n\sum_{l={\ell_o}_i}^{\ell_i-1}\xi^*(l/\rho_i)$. We notice that at least for one agent ($x_o$), the addition to the sum is zero.
Following definition, for all $i,\ell$, s.t. $1\leq i\leq n,\ {{\ell_o}_i} \leq \ell \leq \ell_i-1$, $\ell_o/\rho_o<{{\ell_o}_i}/\rho_i$ and also $\ell_o/\rho_o<{\ell}/\rho_i$
Therefore $ord(\ell_o/\rho_o)\geq ord({{\ell_o}_i}/\rho_i)+1$ and also $ord(\ell_o/\rho_o)\geq ord({\ell}/\rho_i)+1$.
Following definition of $\xi$, $\xi(\ell_o/\rho_o)/\xi({{\ell_o}_i}/\rho_i)\geq (k\cdot n)$ and therefore $\xi^*(\ell_o/\rho_o)/\xi^*({{\ell_o}_i}/\rho_i)\geq (k\cdot n)$. Since sum contains at most $(n-1)\cdot k$ non zero items, we conclude that $\delta_o(\ell_o+1)>C_2$.

Next we show that $C_1'-\delta_o(\ell_o+1)\geq C_1$.
Since $\forall{1\leq i\leq n}$,
$\ell'_i/\rho_i > \ell_o/\rho_o$, the value of $C_1'=\sum_{i=1}^n\reward_i({\ell'_o}_i)$ is the maximum possible value for each element in the sum.
Following definitions, ${\ell_o}_o=\ell_o$ and ${\ell'_o}_o=\ell_o+1$ and therefore  
$\reward_i({\ell'_o}_i)-\reward_i({\ell_o}_i)=\delta_o(\ell_o+1)$.
Therefore $C_1\leq C_1'-\delta_o(\ell_o+1)$ and given that we showed that $C_2<\delta_o(\ell_o+1)$ we conclude that $C_1'>C_1+C_2$.

Finlay, since $C_1'>C_1+C_2$ and since $C_1+C_2=\totreward(\mbsoln)$, $\mbsoln$ is not maximizing $\totreward(\cdot)$. a contradiction.


